Situated Understanding of Errors in Older Adults' Interactions with Voice Assistants: A Month-Long, In-Home Study

Our work addresses the challenges older adults face with commercial Voice Assistants (VAs), notably in conversation breakdowns and error handling. Traditional methods of collecting user experiences-usage logs and post-hoc interviews-do not fully capture the intricacies of older adults' interactions with VAs, particularly regarding their reactions to errors. To bridge this gap, we equipped 15 older adults' homes with smart speakers integrated with custom audio recorders to collect "in-the-wild" audio interaction data for detailed error analysis. Recognizing the conversational limitations of current VAs, our study also explored the capabilities of Large Language Models (LLMs) to handle natural and imperfect text for improving VAs. Midway through our study, we deployed ChatGPT-powered VA to investigate its efficacy for older adults. Our research suggests leveraging vocal and verbal responses combined with LLMs' contextual capabilities for enhanced error prevention and management in VAs, while proposing design considerations to align VA capabilities with older adults' expectations.

==> Supplementary_materials.tex <==

\section{Findings}
\subsection{Multi-Turn Conversations}
\label{app:findings-multi-turn}
To identify whether participants engaged in multi-turn conversations, we grouped single user query-VA response pairs into multi-turn interactions %\cmh{still do not understand. clear now?? Asked others, it is clear to them}, 
provided the topic remained the same or the participant continued the interaction with the VA; potential multi-turn conversations were identified from recorded audio interactions.

Upon analyzing interactions that were contiguous and centered around the same topic---such as sequences of back-and-forth questions---we identified a substantial number of true multi-turn interactions.
%upon grouping interactions that were contiguous and maintained the same topic---such as multiple back-and-forth questions---we discovered a significant number of multi-turn interactions. 
The continuity in conversations was effectively captured by our recording device, which also aided in discerning if participants had purposefully continued the interaction. Although the majority of interactions (out of 2,552 total turns) were single-turn ($n$ = 1,173), a substantial number involved more than one turn, with 348 instances of two-turn interactions.
Out of the total 2,552 turns, we identified 1,379 instances %(1173 + 348 + \dots) 
%\cmh{this number does not seem to match Fig. 3. NOW IT DOES} 
as being part of multi-turn interactions. Fig. \ref{fig:multi-turn} illustrates the number of turns in these interactions and their frequency. 

\begin{figure*}[t]
     \includegraphics[width=\textwidth]{figures/multi-turns-in-interactions.pdf}    
     \caption{2,552 total one-turn interactions, 1,379 ($348\times2+57\times3+\dots$) of which were additionally part of multi-turn interactions.}
    
    \label{fig:multi-turn}
\end{figure*}

\subsection{Trends in VA Usage Over Time}
\label{app:findings-usage}
Most of our findings regarding participants' usage patterns confirm prior work \cite{pradhan2020use, kim2021exploring}; below, we provide a comprehensive overview of user engagement with the VA, highlighting any usage trends that emerged over time.
%we present our findings on features of VA that the participants used and how their usage changed over time.  

%\subsection{Older Adults' Usage Patterns: Changes Across Participants}
%\subsubsection{Features in use}

%In our study, we analyzed the types of interactions older adults have with Alexa, a voice assistant, categorizing them based on the nature of the interaction as shown in Table \ref{tab:interaction_categories}. 
%We coded type of interaction for each turn as informed from prior work \cite{pradhan2020use, kim2021exploring}. 
%Interactions were primarily functional ($n=1130$), aiding in memory-related tasks like reminders, timers, calendar updates, and list creation, as well as inquiring about weather and Alexa's capabilities. Entertainment uses ($n=753$), particularly music and radio, were also prevalent. Some participants also engaged Alexa for jokes, stories, and poems. Our findings align with existing literature on older adults' usage of smart speakers \cite{arnold2022does}. 

%The most frequent interaction type was question-asking ($n=414$), primarily for information seeking. These inquiries were further categorized (see Table \ref{tab:question-type}) to understand the nature of information sought \cite{pradhan2020use}, with entertainment-related questions ($n=98$) being the most common. Participants also queried about Alexa itself; for instance, ``how old are you?'' and ``are you a spy?''. 
\subsubsection{Features in use}
\label{sec:findings-features-in-use}
We analyzed the types of interactions older adults had with Alexa and categorized them based on the nature and goal of the interaction as shown in Table \ref{tab:interaction_categories}. 
%We coded type of interaction for each turn as informed from prior work \cite{pradhan2020use, kim2021exploring}. 
Interactions were primarily functional ($n=1130$), aiding with memory-related tasks like reminders, timers, calendar updates, and list creation, as well as inquiries about the weather and Alexa's capabilities; for instance, P15 regularly set reminders for her nightly medication and occasionally queried Alexa to confirm if she had taken her medication or not. Entertainment uses ($n=753$), particularly involving music and radio, were also prevalent. Some participants additionally engaged Alexa for jokes, stories, and poems. 
The most frequent interaction type was question-asking ($n=414$), primarily for the purpose of seeking information; these inquiries were further categorized (see Table \ref{tab:question-type}) to understand the nature of the information sought \cite{pradhan2020use}, with entertainment-related questions (\eg \textit{``Is the Orioles game televised today?''} and \textit{``When was the children's book} Room on the Broom \textit{published?''}) %\cmh{what would be an entertainment question?} 
being the most common ($n=98$). Participants also queried Alexa about itself (\eg \textit{``How old are you?''} and \textit{``Are you a spy?''}).
%Table \ref{tab:alexa-dialogue-questions} \cmh{fix reference }has example conversations of such interactions. 
Our findings align with existing literature on older adults' use of smart speakers \cite{arnold2022does}. \\
%ammari2019music for younger adults
\textbf{Features in use across participants.}
The frequency and nature of interactions varied among participants, as illustrated in Fig. \ref{fig:interaction_categories}. Notably, P5 and couple P10 found limited utility in the device; for example, P5 remarked, \textit{``I couldn't think of ways to use it \dots Maybe I'm not too creative a thinker,''} while P10's usage was affected by one of the pair's full-time employment: ``\textit{Really, I get done with my work day and I really don’t have the time and energy to go exploring new things \dots I’m comfortable interacting with computers, and this was just a new thing that I have to learn that, as I said, I didn't find additional utility in.''}
In contrast, P15 heavily used Alexa for functional tasks, logging 359 interactions---most notably for medication reminders; P15 regularly set reminders for her nightly medication and occasionally queried Alexa to confirm whether she had taken her medication. Entertainment was the second-most frequent use overall, with P3 executing 138 interactions in this category, mostly to listen to music ($n=119$). Participants also exhibited diverse information-seeking behaviors; for instance, P2 had 130 interactions ranging from inquiries about celebrities to probability questions; C1 in Table \ref{tab:alexa-dialogue-errors} provides an example. Additionally, some participants explored more features than others; for instance, P15 wanted to connect her Audible account with Alexa to listen to audiobooks and she also synced her personal calendar to the smart speaker to get audio notifications.


Participants' social interactions with Alexa (\eg expressing gratitude or greeting the device) varied. While some (\eg P6, P15) frequently thanked or greeted Alexa, others (\eg P1, P7, P9, P12) did not engage in such social customs; this variance may reflect differing perceptions of Alexa as a tool versus a social entity. In particular, we observed that P15 used a social response (\eg ``Thank you'') instead of a command (\eg ``Stop'') for her reminders, suggesting a preference for more socially ``polite'' interactions with the device \cite{pradhan2019phantom}.


Couples P12 and P1, who owned multiple smart speakers, showed a more fixed pattern of usage; as documented in Table \ref{tab:tech-use}, they primarily used Alexa for entertainment and functional tasks such as setting timers ($n=22)$ and communication ($n=27)$, with limited experimentation in other functionalities. Interestingly, despite not mentioning this use in their pre-study interviews, they also engaged in information-seeking activities ($n=27$). Similarly, P12 primarily utilized Alexa for entertainment---predominantly for listening to the radio ($n=44$)---and for communication purposes ($n=9$) without exploring additional functionalities.


%TC:ignore
\begin{comment}
    
\begin{table}[tb]
\centering
\caption{Example conversations of question type of interactions ``\dots'' represents truncation of conversation for brevity.  Full conversations are presented in supplementary materials. `CX' is the tag used to refer to the conversations}
\label{tab:alexa-dialogue-questions}
\begin{tabular}{p{0.3cm} M L}
%\hline
\textbf{Tag} & \textbf{Participant} & \textbf{Alexa} \\
\midrule
\midrule


C2 \newline P2& Alexa I've got a math problem what is the likelihood today June the twenty fourth that I will get one hour straight sun?
& In [city], at 11:00 AM, it'll be 76 degrees Fahrenheit with cloudy skies. At 12:00 PM, \dots \\ %it'll be 78 degrees with cloudy skies. At 1:00 PM, it'll be 80 degrees with cloudy skies. At 2:00 PM, it'll be 80 degrees with thunderstorms and mostly cloudy skies.  \\ 
\cdashline{2-3}
 & Alexa you did not answer the math question the answer should come in percentage &  In [city], at 11:00 AM, it'll be 76 degrees Fahrenheit with cloudy skies. At 12:00 PM,  \dots \\ % it'll be 78 degrees with cloudy skies. At 1:00 PM, it'll be 80 degrees with cloudy skies. At 2:00 PM, it'll be 80 degrees with thunderstorms and mostly cloudy skies. \\
\hline

%\multirow{2}{*}{Tag2} & Conversation4 & Pattern4 \\
%\cline{2-3}
%& Conversation5 & Pattern5 \\
%\hline
\end{tabular}
\end{table}
%TC:endignore
\end{comment}

 \begin{figure*}[h]
     \includegraphics[width=\textwidth]{figures/type-of-interaction-participant.pdf}    
     \caption{Types of interactions for each participant.}
    
    \label{fig:interaction_categories}
\end{figure*}


%In appendix
%The frequency and nature of interactions varied among participants, as illustrated in Fig. \ref{fig:interaction_categories}. Notably, P5 and a couple (P10) found limited utility in the device (P5 said, ``\textit{I couldn't think of ways to use it\dots Maybe I'm not too creative a thinker}''), with the latter's usage impacted by the husband's full-time employment (P10 mentioned, ``\textit{Really I get done with my work day and I really don’t have the time and energy to go exploring new things\dots I’m comfortable interacting with computers, and this was just a new thing that I have to learn that as I said I didn't find additional utility}'').
%In contrast, P15 heavily relayed functional tasks to Alexa, logging 359 interactions, notably for medication reminders. We noted that P15 regularly set reminders for her nightly medication and occasionally queried Alexa to confirm whether she had taken her medication. Entertainment was the second most frequent use, with P3 having 138 interactions in this category, mostly for music ($n=119$). Participants also exhibited diverse information-seeking behaviors; for instance, P2 had 130 interactions, ranging from inquiries about celebrities to probability questions. Table \ref{tab:alexa-dialogue-questions} AC1 and C2 are example conversations. Some participants explored more features than others such as P15 wanted to connect their audible to Alexa to listen to audiobooks. She also synced her personal calendar to Alexa to get notifications. 

%Moreover, couples P12 and P1, who owned multiple smart speakers, showed a more fixed pattern of usage. As documented in Table \ref{tab:tech-use}, they primarily used Alexa for entertainment and functional tasks such as setting timers ($n=22)$ and communication ($n=27)$, with limited experimentation in other functionalities. Interestingly, despite not mentioning it in their pre-study interviews, they also engaged in information-seeking activities using Alexa ($n=27$). Similarly, P12 primarily utilized Alexa for entertainment, predominantly listening to the radio ($n=44$), and for communication purposes ($n=9$), without exploring additional functionalities.









\subsubsection{Usage over time}

\label{app:findings-usage-over-days}

%supports prior work

In examining VA usage trends over time, we considered interaction categories to simplify our analysis (see Fig. \ref{fig:uagaes-over-days}). \\
\textbf{From exploratory behavior to selective use.} %\cmh{unsure how to interpret this heading. From exploratory ... to ...}} 
A notable observation is a decline in overall usage over time, which is consistent with prior work \cite{pradhan2020use, lopatovska2019talk}; participants' initially high usage, characterized by exploratory behavior as the participants experimented with various features, gradually settled into a pattern of utilizing select features that were found to be beneficial in their daily lives. Prior work has discussed factors influencing such a decline in use, including usability issues, forgetting the wake word, and perceived discomfort when talking to a ``machine'' \cite{pradhan2020use}. \\
%evolving user preferences. % [ADD QUOTES ON WHY PEOPLE STOP USING OVER TIME]. 
%%new findings
\textbf{Usage variation across interaction categories.} While looking at the purpose of VA interactions, we found that functional interactions remained the most consistent category over the four-week period, even despite a gradual decline; as functional interactions are need-driven and support daily activities, they tend to integrate more seamlessly into users' routines. In contrast, entertainment-oriented interactions such as listening to music, playing the radio, or asking for jokes exhibited more variability; these desire-driven interactions may be influenced by factors such as mood, available leisure time, and personal preferences, leading to their inconsistent frequency. \\
\textbf{Usage spikes during experimenter check-ins and ChatGPT deployment phase.} Interestingly, we observed spikes in collective usage during specific periods, such as the Week 1 check-in with the experimenter and the ChatGPT deployment phase. These instances suggest that indirect reminders of the VA's presence can temporarily boost usage, although this effect diminishes quickly (as evidenced by the usage peaks in Fig. \ref{fig:uagaes-over-days}).
During the ChatGPT deployment phase, we noticed a spike in usage that can be attributed to participants exploring the new feature; this phase also saw an increase in information retrieval requests using Alexa, possibly for two reasons: 1) failure to activate the ChatGPT skill (\ie forgetting to use the ChatGPT activation phrase ``Let's talk''), resulting in the system defaulting to querying Alexa, %\cmh{still not following the logic here}, 
and/or 2) this phase reminded participants of Alexa's capabilities in answering questions and providing information. 


Usage trends over time varied per participant, as well (see Fig. \ref{fig:uagae-over-days-participant}). 
For example, P5 and couple P10 discontinued their use of the device, finding it unhelpful; conversely, some participants---such as P15, P6, and couple P11---engaged with Alexa more consistently, while others like P2 and P3 demonstrated fluctuating patterns of use, with some days seeing more interaction than others.



%The usage trend over days varies for participants as well (see Fig. \ref{fig:uagae-over-days-participant}). P5 and the couple P10 discontinued usage, finding the device unhelpful. Conversely, some participants such as P15, P6, and the couple P11 engaged with Alexa more consistently. While others such as P2 and P3 demonstrated fluctuating patterns of use, with some days seeing more interaction than others.




\subsubsection{Usage at different times of day}

When examining the cumulative four-week data, we analyzed the hours of the day during which users interacted most with Alexa, illustrated in Fig. \ref{fig:uagae-over-hours}. Consistent with previous research \cite{kim2021exploring}, we identified three primary usage peaks: around 8 a.m. (morning), 12 p.m. (noon), and 6 p.m. (evening/night).
%Notably, the evening-night peak exhibited a more spread-out pattern, indicative of varying spare time and night routines among users. This variability is further evidenced by some interactions occurring as late as 1 a.m., reflecting diverse user schedules.
%Furthermore, we observed that functional interactions were more evenly distributed throughout the day compared to entertainment and information-seeking interactions suggesting that functional tasks, being integral to daily routines, are more consistently engaged with at various times. In contrast, entertainment and information-seeking activities showed more concentrated peaks, likely reflecting periods of leisure or specific needs.
Interactions related to the exploration of ChatGPT were predominantly confined to the afternoon, indicating that users tended to experiment with this feature in their spare time, possibly when other commitments were less pressing.

Usage patterns varied across participants, following the findings of prior work \cite{pradhan2020use}; detailed results are presented in Appendix \ref{app:findings-usage}. 



 \begin{figure*}[t]
     \includegraphics[width=1.12\textwidth, trim={2.7cm 0 0 0},clip]{figures/usage-over-days.pdf}    
     \caption{Interaction categories and their changes in usage over time averaged over all participants.}
    
    \label{fig:uagaes-over-days}
\end{figure*}





 \begin{figure*}[t]
     \includegraphics[width=\textwidth]{figures/usage-over-hours-of-days.pdf}    
     \caption{Interaction categories and their changes in usage over 24 hours averaged over four weeks.}
    
    \label{fig:uagae-over-hours}
\end{figure*}






%\label{app:usage-over-days}

%In analyzing the usage trends of Alexa over time, we considered interaction categories to simplify the analysis (see Fig. \ref{fig:uagaes-over-days}). 
%A notable observation is the decline in overall usage with time. The initial high usage, characterized by exploratory behavior where participants experimented with various features, gradually settled into a pattern of utilizing select features they found beneficial in daily life. Factors influencing this decline include usability issues, system breakdowns, and evolving user preferences. % [ADD QUOTES ON WHY PEOPLE STOP USING OVER TIME]. 



%Interestingly, we observed spikes in collective usage during specific periods, such as the week 1 check-in with the experimenter and the ChatGPT deployment phase. These instances suggest that indirect reminders of the device's presence can temporarily boost usage, although this effect diminishes quickly (as evidenced by the usage peaks in Fig. \ref{fig:uagaes-over-days}).
%During the ChatGPT deployment phase, we noticed a spike in activity, that can be attributed to participants exploring this new feature. This phase also saw an increase in information retrieval interactions, for two primary reasons: 1) failed attempts to activate the skill, leading to direct conversations with Alexa, and 2) a renewed awareness of Alexa's capabilities and its potential to answer queries



%Functional interactions, despite a gradual decline, remained the most consistent category over the four-week period. Since these interactions are need-based and support daily activities, they tend to integrate more seamlessly into users' routines. In contrast, entertainment-oriented interactions, such as listening to music, radio, or asking for jokes, showed more variability. These want-based interactions may be influenced by factors such as mood, available leisure time, and personal preferences, leading to their inconsistent frequency.





 \begin{figure*}[t]
     \includegraphics[width=\textwidth]{figures/usage over days participants.pdf}    
     \caption{Changes in participant usage for each day over four weeks.}

    
    \label{fig:uagae-over-days-participant}
\end{figure*}


%\subsubsection{Usage over times of days}
%\label{app:usage-over-times-of-days}
%In examining the cumulative four-week data, we analyzed the hours of the day during which users interacted with Alexa, as illustrated in Fig. \ref{fig:uagae-over-hours}. Consistent with previous research \cite{kim2021exploring}, we identified three primary usage peaks: around 8 a.m. (morning), 12 p.m. (noon), and 6 p.m. (evening-night). Notably, the evening-night peak exhibited a more spread-out pattern, indicative of varying spare time and night routines among users. This variability is further evidenced by some interactions occurring as late as 1 a.m., reflecting diverse user schedules.

%Furthermore, we observed that functional interactions were more evenly distributed throughout the day compared to entertainment and information-seeking interactions suggesting that functional tasks, being integral to daily routines, are more consistently engaged with at various times. In contrast, entertainment and information-seeking activities showed more concentrated peaks, likely reflecting periods of leisure or specific needs.
%Interactions related to the exploration of ChatGPT were predominantly confined to the afternoon, possibly indicating that users tended to experiment with this feature during their spare time, possibly when other commitments were less pressing.
\subsection{The Social Nature of Voice Interactions }
\label{app:findings-social}
Our audio recordings uncovered new social aspects of VA interactions extending beyond typical use not regularly captured in usage logs; our recordings provide a more situated understanding of users' interactions with the VA and the VA's presence in their daily lives.
%Our audio recordings revealed social aspects of interactions beyond typical VA usage. Such aspects, while can augment the situated understanding of users' interactions with VA, are not usually captured in usage logs otherwise. 


\subsubsection{Social responses and reactions}
\label{sec:social-responses}
Our analysis revealed that participants' interactions with Alexa also included social responses, as detailed in Table \ref{tab:social-responses}. These interactions extended beyond mere task completion. \\
\textbf{Valence of social interactions.} Participants  %often\cmh{compared to the no category, these reactions are not really often.} 
expressed gratitude ($n=179$, \eg ``Thank you''), greeted Alexa ($n=14$, \eg ``Good morning,'' ``Good night,'' etc.), and laughed ($n=13$) at its responses. Additionally, some participants ascribed human characteristics to Alexa because of the way it responded to social interactions, as P14 mentioned: \textit{``When I say, `Thank you, Alexa,' Alexa will say, `Oh, you are welcome, I'm here to serve you.' I don't know why I like to hear that, as if it's a real person or something.''}
We also observed verbal backchannel acknowledgements ($n=20$, \eg ``hmm,'' ``okay'') and participants expressing both positive and negative feedback (backchannel exemplification); positive examples included exclamations of wonder such as \textit{``Isn't that amazing?''} and direct compliments like \textit{``Alexa, I really like you,''} whereas negative feedback was sometimes expressed sarcastically (\eg \textit{``Hell of a job''}) or via critical remarks (\eg \textit{``Alexa is much more stupider''}).
In 21 cases, participants also commented on Alexa's responses or actions (see AC1 and AC2 in Table \ref{tab:alexa-dialogue-private-conversations}).\\
\textbf{Variance across participants.} Participants' social interactions with Alexa varied; while some (\eg P6, P15) frequently thanked or greeted Alexa, others (\eg P1, P7, P9, P12) did not engage in such social customs. This variance may reflect differing perceptions of Alexa as either a tool or a social entity, or it may simply reflect the individual personalities of the participants. \\ %\cmh{or might be just the participant's personality}. \\
\textbf{Social responses as implicit methods of communication.} An interesting observation occurred when P15 used a social response (\ie ``Thank you'') instead of a command (\ie ``Stop'') with her reminders, suggesting a preference for more socially ``polite'' interactions with the VA---a phenomenon also highlighted by prior work \cite{pradhan2019phantom}. Another illustrative example occurred in C12 (Table \ref{tab:alexa-dialogue-errors}), when P15 responded naturally (\eg \textit{``I took my medicine''}) to a ringing reminder to cancel it, but failed to achieve this result. Using a social or natural response instead of a direct command further underscores the tendency of certain individuals to apply implicit communication cues akin to those used in human interactions in their interactions with VAs. Similar behavior was also evident when participants expressed gratitude to the VA even when it failed to fulfill their request, as illustrated in Table \ref{tab:errors-reactions}. The implicit, natural methods of communication used by participants suggest that they may attribute social characteristics to VAs, thus influencing the nature of their communications with them; however, we observed that Alexa often failed to comprehend such implicit communication methods (see C12) even as participants continued to use them, indicating a mismatch between participants' mental models of the VA's capabilities and its actual functionalities.


%\subsubsection{Other social dynamics}
\subsubsection{VAs in social conversations}
\label{sec:social-dynamics}

In our study, we not only observed users' social responses and reactions to Alexa during their interactions with it, but also identified social conversations about Alexa that lent additional insight into the extent of the VA's integration into its users' lives (Table \ref{tab:other-aspects}, left). As examples, we captured participants' discussions about Alexa, instructional conversations on its use, and dialogues stemming from topics initiated with the VA.
Notably, participants typically talked about Alexa ($n=50$) either immediately after or during its use, as depicted in AC3 in Table \ref{tab:alexa-dialogue-private-conversations}.

Additionally, there were 21 instances where participants engaged in discussions on how to operate Alexa with others---more frequently couples trying to navigate its functionality together (C9, Table \ref{tab:alexa-dialogue-private-conversations}) and less frequently when participants were showcasing Alexa to visitors (AC4, Table \ref{tab:alexa-dialogue-private-conversations}).
Participants also engaged in conversations related to topics initiated with Alexa, highlighting the VA's primarily need-based usage and indicating a deeper integration of the system into their daily lives. An illustrative example may be found in couple P11's discussion of the history of Tony Bennett, in which P11a relied on Alexa for information only to find that it did not provide the expected response (C8, Table \ref{tab:alexa-dialogue-private-conversations}); another example occurred in AC5 (Table \ref{tab:alexa-dialogue-private-conversations}), when P1a verified Alexa's answer to P1b's question.



%\subsubsection{Potential negative social interactions}
\subsubsection{Social indicators of friction}
As previously highlighted in Section \ref{sec:error-reactions}, Alexa elicited verbal reactions of a social nature when conversational breakdowns occurred as a result of one or more errors. The elicited social reactions ranged from acknowledgement and laughter to negation and negative commentary to even positive remarks and expressions of gratitude, as detailed in Table \ref{tab:errors-reactions}. Such a diverse array of social responses suggests that participants' interactions with the VA extended beyond mere transactional exchanges.

In addition to reactions to errors, we also captured and coded aspects of participants' interactions that indicated friction in their conversations and that would not typically be captured by usage logs---for instance, interruptions and overlap in both Alexa's and the participants' speech (Table \ref{tab:other-aspects}, right). It is worth noting that most of the interruptions in all the collected interaction data (21 out of 31, as referenced in Tables \ref{tab:errors-reactions} and \ref{tab:other-aspects}) were a direct result of errors made by Alexa.
Despite encountering issues during interactions and the VA's erroneous tendencies as discussed in Section \ref{sec:errors}, our observations revealed minimal overlap and interruptions in participants' speech when interacting with Alexa, suggesting a degree of patience and forgiveness %\cmh{do young adults have this level of patience? something that I have seen is wllingness to work with VA is more in elderly despite more errors than younger adults, that can be reflective of more forgiving behavior} 
toward the VA despite conversational failures. Prior work also reflects a similar sentiment in elderly users---\ie despite experiencing more errors, elderly users tend to exhibit a higher willingness to continue working with voice-based agents in the future as compared to younger adults \cite{barros2020usability}.



%TC:ignore
\begin{table}[t]
    \centering
    \caption{Users' social responses and reactions to Alexa.}
    \label{tab:social-responses}
    \begin{tabular}{lr|lr}
        \toprule
        \textbf{Social Response/Reaction} & \textbf{Count} &\textbf{Social Response/Reaction} &\textbf{Count} \\
        \midrule
        \midrule
        ``No''                                      & 2301 & Greeting                                  & 14 \\
        Gratitude                               & 179  & Laughter                                  & 13 \\
        Remarks                                 & 21   & Verbal backchannel exemplification, negative & 12 \\
        Verbal backchannel acknowledgement      & 20   & Verbal backchannel exemplification, positive & 9  \\
        \bottomrule
    \end{tabular}
\end{table}
%TC:endignore


%TC:ignore
\begin{table}[tb]
\centering
\caption{Conversations exemplifying social aspects beyond simple interactions. ``\dots'' represents the truncation of a conversation for brevity. Full conversations are available in the supplementary materials.}
\label{tab:alexa-dialogue-private-conversations}
\begin{tabular}{p{0.3cm} M L}
%\hline
\textbf{Tag} & \textbf{Participant} & \textbf{Alexa} \\
\midrule
\midrule

AC1 & Alexa, what is Donald Trump's educational background? & Donald Trump was educated at UPenn. \\ %University of Pennsylvania.	\\
\cdashline{2-3}
P2 & \myc{[remarking]} That's it, no Harvard, no Yale. & \myc{[Not heard by Alexa]} \\
 \hline
AC2 & \myc{[User initiates incomplete reminder request.]} & When should I remind you? \\% and is closely related to Chikungunya, O’nyong-nyong, Ross River, Barmah Forest, and Sindbis viruses (1–3). \\
 \cdashline{2-3}
P11b & \myc{[No user response]} & What's the reminder for? \\
 \cdashline{2-3}
 & She remembers it! & \\%, James Biden, and Valerie Biden Owens, and his relative is Valerie Biden Owens. \\
 \hline
AC3 & Alexa, put hard candy on my shopping list.  & You already have hard candy on your shopping list. \\ %University of Pennsylvania.	\\
\cdashline{2-3}
P6 & Oh. \myc{[To visitor:]} Did you hear her? I said, ``Alexa \dots &  \\
 \hline
%C9 & Alexa, give me a 10 minute warning please.  & 10 minutes, starting now \myc{[it worked]} \\ %University of Pennsylvania.	\\
%\cdashline{2-3}
%P11a & & \cellcolor{user} \myc{[P11b to P11a:} No you need to say timer for 10 minutes \myc{[overlapping Alexa speech]}  \\
%\cdashline{2-3}
% & What wait wait what \{P11b's name\} & \cellcolor{user} \myc{[P11b to P11a]:} Set a time for 10 minutes  \\
% \cdashline{2-3}
% & Okay \myc{[To P11b]} Alexa, set timer for 10 minutes & Second timer, 10 minutes, starting now \\
% \cdashline{2-3}
% & Set a time for 10 minutes \myc{[P11b to P11a]} & \\
% \hline
AC4 & Alexa, add milk to my shopping list.  & I added milk to your shopping list. \\ %University of Pennsylvania.	\\
\cdashline{2-3}
P8 & I don't know where the list is. \myc{[Visitor to P8:]} Oh wait a minute, maybe it's in Amazon \dots  &  \\
 \hline
%C8 & Alexa play the history of Tony Bennett.& \cellcolor{user} \myc{[P11b to P11a]:} What's the history of Tony Bennett  \\
%\cdashline{2-3}
% P11a & \myc{[To P11b]} Oh she'll tell you & \cellcolor{user} \myc{[P11b chuckles mockingly]} \\
 \cdashline{2-3}
% & She didn't tell you \myc{[to P11b]}  & \cellcolor{user} \myc{[P11b to P11a]:} Because it makes no sense\\
 \hline
 AC5 \newline P1b & Did the actress who played the voice of Howard Wolowitz on \textit{3rd Rock from the Sun} really die? & From fun107.com: But sadly, the actress behind that memorable voice has passed away. \\
\cdashline{2-3}
 & \myc{[P1a to P1b:]} That is true. She did pass away.  & \\
 \hline
 AC6 \newline P15 & Alexa, tell me a joke. & Sometimes people ask me if I speak lizard. I don't, but iguana learn someday! \\
\cdashline{2-3}
 & \myc{[laughter]} Okay, so you're still working.  & \myc{[Not heard by Alexa]} \\
 \hline

\end{tabular}
\end{table}
%TC:endignore

%TC:ignore
\begin{table}[t]
    \centering
    \caption{Additional aspects of participants' interactions with Alexa.}
    \label{tab:other-aspects}
    \begin{tabular}{lr|lr}
        \toprule
        \textbf{Description }& \textbf{Count} &\textbf{Description} &\textbf{ Count} \\
        \midrule
        \midrule
        Private conversation about Alexa & 50 & Overlap: Participant starts talking over Alexa & 12 \\
        Private conversation about how to use Alexa & 21 & Overlap: Alexa starts talking over participant & 4 \\
        Private conversation about same topic & 15 & Participant interrupts Alexa & 31 \\
        &  & Alexa interrupts participant & 15  \\
        \bottomrule
    \end{tabular}
\end{table}
%TC:endignore
\begin{comment}
    
%TC:ignore
\begin{table}[tb]
\centering
\caption{Additional illustrative conversations.  ``\dots'' represents truncation of conversation for brevity.  }
\label{tab:alexa-dialogue-additional-appendix}
\begin{tabular}{p{0.3cm} S X}
%\hline
\textbf{Tag} & \textbf{Participant} & \textbf{Alexa} \\
\midrule
\midrule

AC6 \newline P15 & Alexa tell me a joke & Sometimes people ask me if I speak lizard. I don't, but iguana learn someday! \\
\cdashline{2-3}
 & \myc{[laughter]} Okay, so you still working  & \myc{[not listened by Alexa]} \\
 \hline


\end{tabular}
\end{table}
%TC:endignore
\end{comment}

%\subsection{Additional Error Analysis}

\begin{figure*}[t]
     \includegraphics[width=\textwidth]{figures/errorneous-interactions.pdf}    
     \caption{For each interaction type, the percentage of interactions that resulted in errors and the percentage of interactions in which the error was resolved or not. Interaction types are listed in descending order of their frequency in the interaction data. The number of errors on each bar indicates the total errors in that interaction type. For instance, 414 interactions were of the ``question'' type; 176, or $44\% (34\%+9\%)$ of those resulted in an error; and only $9\% $ of the 414 interactions were resolved after the first retry. Note: Not all errors had retries and some errors had multiple retries, as discussed later.}
    
    \label{fig:errorneous-interactions}
\end{figure*}

\section{Discussion}
\subsection{Voice Assistance in Older Adults' Lives} %as a Social Entity}

Our findings corroborate prior studies demonstrating the utility of VAs in the lives of older adults, particularly for supporting memory through functional tasks, providing entertainment, and delivering necessary information \cite{kim2021exploring, pradhan2020use}. 
Our participants explored a variety of features, reflecting the VA's multifaceted role in their lives; for instance, playing music and listening to news indicate potential uses of voice assistance beyond need-based tasks. Many participants also engaged in creating reminders and shopping lists, pointing to a blend of functional and entertainment uses for the VA. Some participants used Alexa for more diverse purposes, such as attempting to connect it with their Audible account to listen to audiobooks, syncing their personal calendar to stay updated, and asking the system to tell jokes, stories, and poems, suggesting that VAs are perceived not merely as tools but also as ``digital companions''---a perspective that differs from that of younger adults \cite{chung2019elderly}.
Our study also revealed the creative ways in which different participants interacted with the VA. For example, P15 demonstrated an inventive approach by asking Alexa to tell a joke to check whether it was working after a malfunction (AC6, Table \ref{tab:alexa-dialogue-private-conversations}); this particular instance illustrates the novel ways in which users may adapt their interactions with VAs, transforming routine troubleshooting into a more interactive and enjoyable experience. Similarly, questions such as \textit{``Alexa, are you there?''} or \textit{``Alexa, are you working?''} show a form of human-agent interaction that resembles a ``checking up on'' behavior. 

Our findings expand on existing knowledge by illustrating how smart speaker-based VAs can become integrated and situated within the daily lives of older adults. 
The social interactions with VAs that we captured reveal significant insights; for example, older adults often engage in social niceties with VAs, such as expressing gratitude or greetings (Section \ref{sec:social-responses}), a finding also supported by prior work \cite{pradhan2019phantom}. 
Our findings also align with prior research demonstrating that older adults are more likely to anthropomorphize a virtual agent, often using courteous language to show gratitude, while younger adults generally view virtual agents as more utilitarian tools, focusing primarily on their convenience \cite{oh2020differences, chung2019elderly}.
Expressions of affection toward Alexa---\eg ``I really like you'' or ``I love you''---not only show an emotional attachment that may result in elevated expectations, but also raise ethical concerns about deception, infantilization, and privacy in terms of the nature and impact of such bonds \cite{sharkey2012granny, wachsmuth2018robots}. Given that older adults are a more vulnerable demographic, it is crucial that AI assistance is designed with these potential repercussions in mind.

Furthermore, the use of VAs in situated conversations and as part of social interactions with others (as shown in Section \ref{sec:social-dynamics}) points to their ever-evolving role. Instances when couples involved Alexa in their discussions (C8 and AC5 in Table \ref{tab:alexa-dialogue-private-conversations}) or participants showcased Alexa to visitors (AC3 in Table \ref{tab:alexa-dialogue-private-conversations}) reflect a perception of VAs as active, social entities. 
%Such conversations are also reflective of their impression and mental model of the VA. For instance, C8 shows how the couple P11 has very different mental model from each other since P11a believes that Alexa will be able to answer his question while P11b seems quite sure of the opposite. C9 is an illustrative example of similar mismatch. 
The changing uses and perceptions of VAs among older adults points to their significant role in daily and social activities beyond basic tasks, raising questions about a role that transcends simple assistance; such a shift calls for more discussion around designing VAs to suit the specific needs and preferences of this demographic while considering both ethical aspects and possible improvements. 

%Similarly, Talk2Care, an LLM-powered VA for older adults, improves health information collection and mental support in scenarios such as symptom reporting and post-surgery follow-ups \cite{yang2023talk2care}. Nevertheless, users expressed expectations beyond patient-provider communication, including better integration of the VA with their healthcare management \cite{yang2023talk2care}.

%\subsection{Opportunities, Limitations and Design Considerations for Voice Assistants}







==> comments.tex <==

[1] \url{https://link.springer.com/chapter/10.1007/978-3-030-22015-0_36}

[2] \url{https://dl.acm.org/doi/abs/10.1145/3441852.3471218}

[3] \url{https://www.tandfonline.com/doi/full/10.1080/17483107.2022.2065369}

[4] \url{https://dl.acm.org/doi/10.1145/3373759}

[5] \url{https://dl.acm.org/doi/abs/10.1145/3359316}

[6] \url{https://dl.acm.org/doi/10.1016/j.chb.2021.106914}

[7] \url{https://dl.acm.org/doi/abs/10.1145/3313831.3376760}

[8] \url{https://link.springer.com/chapter/10.1007/978-3-030-34146-6_14}

[9] \url{https://www.proquest.com/docview/2445992614?pq-origsite=gscholar&fromopenview=true}

[10] \url{https://arxiv.org/pdf/2303.00164.pdf}


\begin{table}[h]
\centering
\caption{Dialogue Interaction with Alexa: Information Seeking}
\label{tab:alexa-dialogue}
\begin{tabular}{p{8cm}|p{8cm}}
\textbf{Participant (P2)} & \textbf{Alexa Response} \\
\toprule
What are Joe Biden's roots? & According to an Alexa Answers contributor: Ireland \\
Alexa that's his lineage I wanna know about his mother and his father & [not listened by Alexa] \\
Alexa tell me about virus family his parents. Transcription error, he actually said: Alexa tell me about Joe Biden's family his parents & From cdc.gov: Mayaro virus (MAYV), the cause of Mayaro fever, is a member of the genus Alphavirus, family Togaviridae, and is closely related to Chikungunya, O’nyong-nyong, Ross River, Barmah Forest, and Sindbis viruses (1–3). \\
Alright Alexa you did a really good job at answering question I did not ask you & [not listened by Alexa] \\
Alexa tell me about Joe Biden's family his mother his father & Joe Biden's children are Ashley Biden, Beau Biden, Hunter Biden, and Naomi Biden. His parent is Jean Biden, his siblings are Francis Biden, James Biden, and Valerie Biden Owens, and his relative is Valerie Biden Owens. \\
Alexa show his mother was a single mother Transcription error, he actually said: Alexa so his mother is a single mother? & From educalingo.com: The definition of single mother in the dictionary is a mother who has a dependent child or dependent children and who is widowed, divorced, or unmarried. \\
Alexa Joe Biden's family was did he have a father than you & Joe Biden's father is Joseph R. Biden Sr.. \\
What did he do? (not listened by Alexa) & \\
Alexa what was Joe Biden senior's educational background and what did he do? & This might answer your question: Joe Biden was educated at Syracuse University and the University of Delaware. \\
Alexa what was Joe Biden's father's background? & Hmm, I don't know that one. \\
Alexa did Joe Biden know his father & Joe Biden's father is Joseph R. Biden Sr.. \\
What what was Joseph F. Biden's educational background? & Before his political career, former Vice President Joe Biden was an attorney. In 1965, he received a bachelor's degree in history and political science from the University of Delaware. In 1968, Biden earned his juris doctors degree from Syracuse University College of Law. \\
Alexa stop I'm talking about Joe Biden's father what was his educational background & Sorry, I don't know that one \\
\hline
\hline
Alexa I've got a math problem what is the likelihood today June the twenty fourth that I will get one hour straight sun
& In Gwynn Oak, at 11:00 AM, it'll be 76 degrees Fahrenheit with cloudy skies. At 12:00 PM, it'll be 78 degrees with cloudy skies. At 1:00 PM, it'll be 80 degrees with cloudy skies. At 2:00 PM, it'll be 80 degrees with thunderstorms and mostly cloudy skies.  \\
Alexa you did not answer the math question the answer should come in percentage & 
In Gwynn Oak, at 11:00 AM, it'll be 76 degrees Fahrenheit with cloudy skies. At 12:00 PM, it'll be 78 degrees with cloudy skies. At 1:00 PM, it'll be 80 degrees with cloudy skies. At 2:00 PM, it'll be 80 degrees with thunderstorms and mostly cloudy skies. \\
\hline
\end{tabular}
\end{table}


\begin{table}[h]
\centering
\caption{Example conversations of  ``\dots'' represents truncation of conversation for brevity.  Full conversations are presented in supplementary materials.}
\label{tab:alexa-dialogue}
\begin{tabular}{p{0.3cm} M L}
%\hline
\textbf{Tag} & \textbf{Participant} & \textbf{Alexa} \\
\midrule
\midrule
C1 & What are Joe Biden's roots? & According to an Alexa Answers contributor: Ireland\\
\cdashline{2-3}
P2 & Alexa that's his lineage I wanna know about his mother and his father & [not listened by Alexa] \\
 \cdashline{2-3}
 & Alexa tell me about virus family his parents. \myc{[Transcription error, he actually said: Alexa tell me about Joe Biden's family his parents] }& From cdc.gov: Mayaro virus (MAYV), the cause of Mayaro fever, is a member of the genus Alphavirus, family Togaviridae, and is closely related to Chikungunya, O’nyong-nyong, Ross River, Barmah Forest, and Sindbis viruses (1–3). \\
 \cdashline{2-3}
 & Alright Alexa you did a really good job at answering question I did not ask you & \myc{[not listened by Alexa]} \\
 \cdashline{2-3}
 & Alexa tell me about Joe Biden's family his mother his father & Joe Biden's children are Ashley Biden, Beau Biden, Hunter Biden, and Naomi Biden. His parent is Jean Biden, his siblings are Francis Biden, James Biden, and Valerie Biden Owens, and his relative is Valerie Biden Owens. \\
 \cdashline{2-3}
 & Alexa show his mother was a single mother \myc{[Transcription error he actually said: Alexa so his mother is a single mother?]} & From educalingo.com: The definition of single mother in the dictionary is a mother who has a dependent child or dependent children and who is widowed, divorced, or unmarried. \\
 \cdashline{2-3}
 & Alexa Joe Biden's family was did he have a father than you & Joe Biden's father is Joseph R. Biden Sr.. \\
 \cdashline{2-3}
 & What did he do? & \myc{[not listened by Alexa]} \\
 \cdashline{2-3}
 & Alexa what was Joe Biden senior's educational background and what did he do? & This might answer your question: Joe Biden was educated at Syracuse University and the University of Delaware. \\
 \cdashline{2-3}
 & Alexa what was Joe Biden's father's background? & Hmm, I don't know that one. \\
 \cdashline{2-3}
 & Alexa did Joe Biden know his father & Joe Biden's father is Joseph R. Biden Sr.. \\
 \cdashline{2-3}
 & What what was Joseph F. Biden's educational background? & Before his political career, former Vice President Joe Biden was an attorney. In 1965, he received a bachelor's degree in history and political science from the University of Delaware. In 1968, Biden earned his juris doctors degree from Syracuse University College of Law. \\
 \cdashline{2-3}
 & Alexa stop I'm talking about Joe Biden's father what was his educational background & Sorry, I don't know that one \\
 \cdashline{2-3}
%\cline{2-3}
%& Conversation3 & Pattern3 \\
\hline
C2 & Alexa I've got a math problem what is the likelihood today June the twenty fourth that I will get one hour straight sun
& In [city], at 11:00 AM, it'll be 76 degrees Fahrenheit with cloudy skies. At 12:00 PM, it'll be 78 degrees with cloudy skies. At 1:00 PM, it'll be 80 degrees with cloudy skies. At 2:00 PM, it'll be 80 degrees with thunderstorms and mostly cloudy skies.  \\ 
\cdashline{2-3}
P2 & Alexa you did not answer the math question the answer should come in percentage &  In [city], at 11:00 AM, it'll be 76 degrees Fahrenheit with cloudy skies. At 12:00 PM, it'll be 78 degrees with cloudy skies. At 1:00 PM, it'll be 80 degrees with cloudy skies. At 2:00 PM, it'll be 80 degrees with thunderstorms and mostly cloudy skies. \\
\hline

%\multirow{2}{*}{Tag2} & Conversation4 & Pattern4 \\
%\cline{2-3}
%& Conversation5 & Pattern5 \\
%\hline
\end{tabular}
\end{table}

P2: ``Alexa what is donald trump's educational background''	

Alexa: Donald Trump was educated at the University of Pennsylvania.	

P2:	``That's it, no Harvard no Yale'' (remark)

and 

Alexa: ``When should I remind you?''	

[No user response]

Alexa: ``What's the reminder for?''

P11b: ``She remembers it!''


P8: ``Alexa add milk to my shopping list''	

Alexa: ``I added milk to your Shopping list.''

Visitor to P8: ``I don't know where the list is. Oh wait a minute may be it's in Amazon.''

Below is an example for couples collaborating to learn how to use Alexa:

P11a:``Alexa, give me a ten minute warning please"	

P11b to P11a: "No you need to say timer for ten minutes" 

Alexa ``10 minutes, starting now''	overlapping P11b {you need to say timer for 10 minutes}

P11a to P11b: ``What wait wait what [P11b]''
	
P11b to P11a: ``Set a time for 10 minutes''

P11b to P11a:  ``okay''

P11a: ``Alexa set timer for ten minutes''	

Alexa: ``2nd timer, 10 minutes, starting now''	


P11a: ``Alexa play the history of Tony Bennett''	

P11b to P11a: ``What's the history of Tony Bennett''

P11a: ``Oh she'll tell you''

P11b: chuckles mockingly 

P11a: ``She didn't tell you''

P11b: ``Because it makes no sense''


listened partial: P3: "what are the interesting a historical event"	"what are the interesting a historical event in 19.." cut off by alexa
"There are countless interesting and significant historical events. Here are a few examples: 1. The signing of the Declaration of Independence in 1776, marking the birth of the United States. 2. The French Revolution in the late 18th century, which brought major social and political changes to France. 3. The Industrial Revolution in the 18th and 19th centuries, transforming societies with technological advancements. 4. The end of World War II in 1945, which reshaped the global landscape and gave rise to the Cold War. 5. The moon landing in 1969, as part of NASA's Apollo 11 mission, showcasing human achievement and exploration. 6. The fall of the Berlin Wall in 1989, symbolizing the end of the Cold War and the reunification of Germany. These are just a few examples, and there are many more fascinating historical events throughout time in various parts of the world."





P11a ``Alexa I understand that you now can do chatGPT, is that correct?"	

P11b to P11a	"you have to do certain commands''
P11b``Okay i have to read it then''
``Alexa what do you know about chatGPT''	
``ChatGPT is an AI-powered chat tool released in November 2022. It uses OpenAI's large language models and continues to evolve via supervised and reinforcement learning techniques.''

P12b:

``Alexa let's chat''	
``Hey! I am an intelligent virtual agent programmed to provide you with the requested information to the best of my ability. What do you wanna know?''	
``What's the best way for to make hard boiled eggs?''	
``searching''
``How do you unwind?''	
``I take a nap''	
``Here it is... To make hard-boiled eggs, follow these steps: 1. Place your desired number of eggs in a saucepan and add enough water to cover them by about an inch. 2. Place the saucepan on the stove over medium-high heat and bring the water to a boil. 3. Once the water is boiling, turn off the heat and cover the saucepan with a lid. Let the eggs sit in the hot water for about 9-12 minutes, depending on the size of the eggs and how well-done you like them. 4. After the desired time has elapsed, carefully drain the hot water from the saucepan and transfer the eggs to a bowl filled with ice water. Let them cool for at least 5 minutes to stop the cooking process. Gently tap the eggs on a hard surface and peel them under running water if needed. This method should give you perfectly hard-boiled eggs with a firm and fully cooked yolk.''
``Thank you Alexa''	
%``Sorry, I don't know about that. Is there something else you would like to know? Try saying echo or chatbot before your question if you are trying to ask ChatGPT something.''	
%``Alexa goodbye''	
%``Goodbye''


P15:earlier conversation:

alexa let's talk

Tap / Routine / Type with Alexa:open chat skill	
Hello! As an intelligent voice assistant my purpose is to provide requested information as accurately as possible. How can I assist you today?	
I'm having trouble falling asleep
	i'm having trouble falling asleep. what can you do to help me cut off by alexa
	Fetching that
What is your favorite food?
	
hmmm
	hmmm ham
	I'll quickly look that up
Sorry, I had trouble doing what you asked. Please try again.
	
i'm having trouble falling asleep i take medicine but it doesn't help what should i use to help me fall asleep
	
Here it is... I'm sorry to hear that you're having trouble falling asleep. Here are a few techniques that might help: 1. Create a bedtime routine: Establish a relaxing routine before bed. This might include activities such as reading a book, taking a warm bath, or practicing deep breathing exercises. 2. Create a comfortable sleep environment: Make sure your bedroom is quiet, dark, and at a comfortable temperature. Use comfortable pillows and a supportive mattress, and consider using earplugs or an eye mask if necessary. 3. Limit exposure to screens: Avoid using electronic devices such as phones, tablets, or computers before bedtime. The blue light emitted by these screens can interfere with your sleep. Instead, engage in activities that promote relaxation. 4. Practice relaxation techniques: Techniques such as progressive muscle relaxation, guided imagery, or meditation can help calm your mind and body before sleep. You can find numerous apps or videos that provide guided relaxation exercises. 5. Limit caffeine and stimulants: Avoid consuming caffeine or other stimulants, such as nicotine or alcohol, especially close to bedtime. These can interfere with your ability to fall asleep. If your sleeping difficulties persist, it may be helpful to speak with a healthcare professional for further guidance.	
Audio could not be understood
	
thank you a lot of good information	
	alexa .. cut off by Alexa
What else can I help you with?
	
why should i keep the room dark	why should i keep the room dark to help with sleep
	searching
alexa why should i keep the room dark to help with sleep
	
Here it is... Keeping the room dark can promote better sleep because darkness signals to your body that it's nighttime and time to rest. Our bodies naturally produce a hormone called melatonin, which helps regulate our sleep-wake cycle. Melatonin production increases in response to darkness and decreases when exposed to light. Exposure to light, especially blue light emitted by electronic screens or bright lights, can suppress melatonin production and interfere with your body's natural sleep signals. By keeping the room dark, you minimize external sources of light that can disrupt your melatonin levels and make it harder for you to fall asleep. Additionally, darkness promotes a more relaxing and soothing environment, which can help your mind and body relax and prepare for sleep. With less visual stimulation, you're more likely to feel calm and at ease, which can make it easier to fall asleep and stay asleep throughout the night. If your room is not naturally dark, you can use light-blocking curtains or blinds to keep out external light sources. It's also a good idea to minimize the use of electronic devices with bright screens in your bedroom, as they can emit unwanted light and disrupt your sleep patterns.
	
ok thank you
	
What else can I help you with?	
ummm nothing else thank you
	
Sorry, I don't know about that. Is there something else you would like to know? Try saying echo or chatbot before your question if you are trying to ask ChatGPT something.	
no nothing
	
	fetching that
Do you have any pets?
	
no no pets
	
Here it is... If you feel that none of the suggestions are helpful or applicable to your situation, here are a few additional techniques you may try to help you fall asleep: 1. Try relaxation exercises: Deep breathing, progressive muscle relaxation, or visualization exercises can help calm your mind and body. Focus on your breathing or imagine yourself in a peaceful and comfortable place. 2. Practice good sleep hygiene: Develop healthy sleep habits such as maintaining a consistent sleep schedule, avoiding naps during the day, and creating a comfortable sleep environment. 3. Avoid stimulating activities before bed: Engage in relaxing activities before sleep, such as reading a book, listening to calming music, or taking a warm bath. Avoid mentally or physically stimulating activities that may make it harder for you to relax. 4. Ensure your sleep environment is comfortable: Make sure your bedroom is at a comfortable temperature, free from excessive noise, and with a comfortable mattress and pillows that suit your preferences. 5. Consider professional help: If your difficulty falling asleep persists or significantly impacts your daily life, it may be beneficial to consult a healthcare professional or sleep specialist who can provide personalized advice and interventions. Remember, everyone's sleep needs are different, and it may take time to discover the techniques that work best for you. It's essential to be patient and persistent in finding a solution that improves your sleep quality.	
alexa stop	interrupted Alexa after {comfortable place 2, } and before{practice good sleep}
Goodbye!	




Good conversation with ChatGPT Alexa skill after few tries in earlier days, smooth. suggests need some practice and simpler ChatGPT interface


``alexa let's chat''

"Hey! I am an intelligent conversational assistant designed to present requested information. What do you wanna know?"
``is the extreme heat ummm natural to weather''

``What's a good book that you have read?''

``ummm god's kingdom come''

"Here you go...Extreme heat is a natural occurrence in weather patterns. It can be caused by various natural factors such as high-pressure systems, heatwaves, or the position of the sun. Additionally, extreme heat can also be influenced by climate patterns such as El Niño or changes in global climate due to factors like greenhouse gas emissions. While natural variability in weather patterns plays a role in extreme heat events, human activities, specifically the emission of greenhouse gases, have contributed to the overall increase in global temperatures. This has led to an increase in the frequency, intensity, and duration of heatwaves and extreme heat events in many parts of the world. It's important to note that climate change is causing shifts in weather patterns and making extreme heat events more frequent and severe. It is necessary to address the underlying causes of climate change and take appropriate measures to mitigate its impact on extreme weather conditions."
``hmmm can you tell me a story''

``Any other questions for me?''

``can you tell me a story''


``What's your favourite way to relax?''

``a nap''


"Here it is... Certainly! Here's a short story for you: Once upon a time, in a small village nestled among rolling hills, there lived a curious young girl named Maya. Maya loved exploring and had a special fondness for the ancient oak tree that stood at the edge of the village. One sunny day, Maya decided to venture deeper into the forest beyond the oak tree. As she walked through the lush greenery, she stumbled upon an old, rusted key lying on the ground. Intrigued, she picked it up, wondering what it might unlock. Driven by curiosity, Maya embarked on a quest to find the mysterious lock that the key would open. She spent days searching every nook and cranny of the village, looking for clues. Finally, an elderly villager named Mr. Andrews noticed Maya's dilemma and shared an old folktale about a hidden treasure in a long-forgotten cave. With newfound hope, Maya followed Mr. Andrews' directions, climbing the hills and navigating through a thick forest until she reached the mouth of a dark cave. The air was cool, and mysterious whispers seemed to echo through the ancient walls. Brave yet cautious, Maya took a deep breath and entered the cave, heart pounding with excitement. Guided by her flickering flashlight, she explored further, until she stumbled upon a treasure chest nestled in a secret chamber. Holding her breath, Maya used the old rusty key. With a satisfying click, the chest creaked open, revealing a brilliant array of gemstones, ancient scrolls, and a handwritten letter. The letter, addressed to her, spoke of wisdom, bravery, and the importance of following one's curiosity. Filled with gratitude and a sense of accomplishment, Maya emerged from the cave, treasure in hand. She realized that the real treasure wasn't the gemstones or ancient artifacts—it was the knowledge she had gained, the friends she made along the way, and the strength that came from pursuing her passions. From that day on, Maya became known not only for her curiosity but also for her courage, inspiring others in the village to embrace their own sense of adventure and pursue their dreams. And so, Maya's story spread far and wide, reminding everyone that sometimes, the greatest treasure awaits those who dare to follow the path of curiosity and explore the unknown."
``ugh thank you good story''
"


"You're welcome! I'm glad you enjoyed the story. If you have any more requests or questions, feel free to ask."
"i have a question what's good music to help me relax"

``How do you unwind?''

"No text stored

``Should I continue?''

``yes''

"Here you go...The choice of relaxing music varies from person to person, as everyone has different preferences. However, here are a few genres and artists known for creating calming and soothing music: 1. Ambient music: Ambient music often has atmospheric soundscapes and minimalistic compositions, which can help create a relaxing and serene atmosphere. Artists like Brian Eno, Stars of the Lid, and Harold Budd are popular in this genre. 2. Classical music: Many classical compositions have a soothing and relaxing effect on the mind. Pieces by composers such as Johann Pachelbel ("Canon in D"), Erik Satie ("Gymnopédies"), and Claude Debussy ("Clair de Lune") are often recommended for relaxation. 3. Instrumental music: Instrumental music, particularly genres like acoustic guitar, piano, or instrumental post-rock, often evokes a calming and tranquil mood. Artists like Ludovico Einaudi, Yiruma, or Sigur Rós are known for their soothing instrumental compositions. 4. Nature sounds: Natural sounds such as rain, ocean waves, or forest sounds can create a peaceful ambiance. You can find recordings or playlists that feature these sounds combined with soft background music for a serene experience. 5. Meditation or relaxation music: Many artists create specific music for relaxation and meditation purposes. Look for artists like Deuter, Steven Halpern, or Karunesh, who specialize in creating music intended for relaxation and stress reduction. Remember, these are just general suggestions, and it's important to explore different genres and artists to find what personally resonates with you and helps you relax. Experiment with different styles and see what music supports your own relaxation and stress relief."
"thank you very expensive information thank you"
``What else can I help you with?''

``nothing right now thank you''

"You're welcome! If you ever have more questions or need assistance in the future, feel free to ask. I'm here to help. Enjoy your relaxation time!"

No text stored

``Any other questions for me?''

"no"

"If that's allGoodbye!"

"goodbye"

``Goodbye!''



%The usage frequency and type varies for participants as shown in Fig \ref{fig:interaction_categories}. P5 stopped using the smart speaker because she did not find much use for it [ADD QUOTE] Similarly, couple P10 did not find much use for the device as well. The husband was employed full time hence was not at home enough and the wife did not see any utility in the device [ADD QUOTE]. All participants used Alexa for functional tasks consistently. However, some participants had much greater use for it. For instance, P15 had 359 functional interactions to support her daily activities such as remembering to take medications. We observed that she put reminder for her night medication every day and would sometimes check in with Alexa to confirm if she took her medication or not. Entertainment, being the second most category of use, is also frequently used by participants such as P3  had 138 entertainment interactions and most of these interactions ($n=119$) were for listening to music. Participants had varied usage behavior for information seeking by asking Alexa various questions. P2 interacted with Alexa 130 times for seeking information about various topics. His questions varied from asking about famous personalities to asking Alexa about probability. Table \ref{tab:alexa-dialogue} shows example conversations. Social interactions (comprising of gratitude and greetings) are usually accompanied with other participant interactions. Some participants tend to say ``Thank you'' or greet Alexa more often (P6 and P15) than others while some do not have such social responses to Alexa at all (P7, P9, P12, P16). Since some people treat Alexa as machine [ADD P9's QUOTE] while others may treat is more socially [FIND QUOTE]. P15 said Alexa thank you instead of Alexa stop when reminder/timers rang indicating that they want more social interaction. [ADD EXAMPLE FROM NOTES]. 

%Another thing to notice across participants is that couples P12 and P16 already owned multiple smart speakers in their home. It can be seen that they have more fixed use for Alexa and do not try other functionalities much; P12 sticks to their entertainment ($n=47$) and functional ($n=14$) use while P16 predominantly use Alexa for functional tasks ($n=72$). As mentioned in their prior technology use in Table \ref{tab:tech-use}, they used it for communication ($n=27)$ and timers ($n=22$). Interestingly, they also used it for information seeking ($n=27$) which is not pointed out by them in their pre-study interview. Similarly, P12 continued using Alexa for entertainment (radio: $n=44$ and communication: $n=9$) and did not experiment with other functionalities. 


\subsection{Notes by Amama}
Interesting observation from field study. People not only respond to Alexa verbally (thank you, okay, I like you Alexa) , non-verbally (laughter, louder tone etc), they also have conversation about it if people are around. For example, a participant was “showing it off” to friends. One of the couples (P11) argue how to use it accurately. P11: They also talk about how their partner is using it wrong while they are interacting. Some quite funny conversations indeed. E.g. husband: she is not clear to me. Wife: no body is (chuckle)
This indicates some form of integration into their lives.  Prior work talks about how people give up using Alexa or use it less over time but we can try to talk about how every time anyone gets new gadget they use it a lot in beginning, explore all kinds of thing, but then the usage drops because they only find few features that they want to or need to use after that initial exploration phase. If we can show that even though usage declines or saturates (not essentially bad thing) over time, people still react in a similar manner to Alexa or around Alexa, it can show integration into their life “getting used to”. So it may not always be abandoning the smart speaker, it may be finding what you want or need it for eventually.

P11 the couple has very different mental models, the husband talks to alexa like a alexa has understanding like a human but the wife treats it as `dumb machine' says everything very systematically, set phrases with details. for instance, she first said: alexa stop and the timer did not once stop for whatever reason then she said alexa stop the timer or cancel the timer and it worked. so she after that mostly always say the whole thing alexa stop/cancel the timer even though Alexa stop would work. On day 11 so far, their mental model is not merging still. 
Husband also have high expectations of Alexa 

H: ``alexa play the history of tony bennett''	

W: ``what's the history of tony bennett''

H: ``oh she'll tell you''

W: chuckles mockingly 

H: ``she didn't tell you''

W: ``because it makes no sense''

Alexa did not respond
The wife had to cancel timer multiple times, so she once said it twice just to be sure even though first time worked



P15-Leslie: ``alexa i'm done i took my medicine'' repeatedly: Alexa had difficulty understanding that the participant did what they wanted to do and kept reminding every hour still. It does only key word stuff cant understand user intent accurately 
Have to say "done" etc..

 ``alexa i took my medicine''  ``Sorry, I don't know that.'' naturally next time says this but Alexa cant comprehend unless says done cancel etc

 Leslie					``alexa i took my medicine''

Alexa					``Sorry, I don't know that.''

Leslie					``yes i took my medicine''

Alexa					``Hmm, I don't know that one.''

Leslie					``cancel medicine''

Alexa					``Leslie, I can’t find medicine, what's the date or time of the event you want to delete?''

Leslie					``cancel the alert''


``ok alexa thank you'' to stop timer, Alexa "My pleasure! Just doin' my job! Hope you had a good week." but did not work had to say "stop" ...
 next time she said "Alexa, stop the timer" instead of more humanlike way of saying ok thank you ---  mental model adjustment

people may naturally use thanky you etc to intend that alarm/timer/reminder should stop but alexa does not recognize that as intent. it requires explicit stop which breaks the flow or adds extra effort for users. For instance, P15 daily, or everytime alomst will initially say more natural phrase to say that she is done or say thank you to want to stop the alarm even though it wont work and then she will have to say stop eventually but next time she would still default to natural cues first. thus, indicating that may be older adults or users in general resort to more natural humanlike speech for even purely functional commands and tasks and VAs should be able to understand that to reduce friction and effort on user's part. users do not often change style of speech for machines unless machines aren't able to do that and they have to. may be one reason for low use and effectiveness of VAs. 

P15: Joke as a way to test device working:

``tell me a joke''

``Sometimes people ask me if I speak lizard. I don't, but iguana learn someday!''

	laughter ``okay, so you still working''


 
P15: chatGPT skill had issue and started talking to Alexa to have conversation but couldn't respond to vague follow ups

She eventually wanted to cancel the reminder cause annoying:

Leslie			wake word		``alexa cancel the reminder''

Alexa					``Leslie, you have 2 reminders.''
''Take my medicine by six o'clock, everyday at 6:00 PM and Take my sleep meds, today at 11:00 PM''
''Which one do you want to cancel?``
Leslie					``cancel medicine reminder''

Alexa					``You don't have any cancel medicine reminders set.''

She tells Alexa for medication still??: "alexa i took my sleep meds"   she wanted to just cancel the medicine reminder once because a couple days later she asked "alexa do i have an alarm for medicine"

even without reminder tell alexa at like 9 am : Leslie		``alexa i took my medicine''

Alexa		``Sorry, I'm not sure about that.''

Leslie					``alexa cancel taking my medicine i took my medicine''

Alexa					``Leslie, I can’t find taking my medicine i took my medicine, what's the date or time of the event you want to delete?''

Leslie					``at nine a.m.''

Alexa					``There's nothing on your calendar starting at 9:00 AM tomorrow.''

she asks whether there is a reminder before setting a reminder:

Leslie					``alexa do i have any reminders''

Alexa					``There are no reminders scheduled.''

Leslie				``thank you''

Alexa					`` Absolutely! Happy to help. Hope you've enjoyed your Monday!''

Leslie					``alexa remind me to take my medicine by six o'clock p.m. today''

Alexa					``Ok, I'll remind you at 6:00 PM.''
''This reminder sounds important. Would you like me to follow up on it until it's completed?``


she likes routine, says ``alexa can you do the wake up routine tomorrow at nine a.m.'' b ut alexa cant do and she says "alexa wake me up tomorrow morning at nine a.m."

she wasn't able to consistently set the alarm to 6 pm for medication, did it on aug 6 for everyday. Alexa should be able to proactively ask the frequency of alarms etc. she always consistently agreed for check in ("This reminder sounds important. Would you like me to follow up on it until it's completed?"), for medicine reminder.

P6 --Mary 

"alexa i'm repeating myself is it going to rain today"  after she asked about it about an hour ago.. indicates she thinks Alexa may have memory

she said: "alexa i love you"

unique ways of saying requests: "give me a wake up call at four o'clock today", "good morning how hot is it going to get today", "alexa play something by mozart for the flute"



P6 also say natural phrases to stop alarm:

Mary					"alexa thank you"
Alexa					``Glad to help! Now go live your best life, just like Barbie! '' '' Hope you had a good Saturday.``

Stop cancel can be seen as interuptive and impolite??

compound actions, user answers and issues next question: "yes alexa add them to my favorites alexa what time do the nationals play today" Alexa doesn't do next action

ask for example of that i something visual....

Mary					"alexa what is a meme"

Alexa					"Internet memes are jokes within Internet culture that have achieved a certain level of celebrity, and are generally recognized and shared independently of their original source material. Noteworthy memes are often sarcastically praised for being dank."

Mary					"can you alexa give an example of a meme"

Alexa					"Here is a meme: What Does This Monster Have to Mourn?"

She has the CNN notifications on and selectively plays the ones she wants. she set up routines, even though it did not exactly do what she thought it would.. checks notifications regulalry.. says "goodmoring" to alexa often

She says ``thank you'' at the end of most interactions---weather, sports information, reminders, etc.

barbie theme

P8 Sally
Alexa really became a hot topic of discussion among friends.

P9 Bob
Pleasantly surprised by Alexa's capability to say that rain is stopping in 25 minutes.

In a single sentence, first attempted to create a timer of 8 minutes but then corrected himself to 9. Alexa successfully picked this up.

Alexa saying (chatGPT) 
"I apologize, but as an AI language model, ....." what does that even mean to older adults or people unaware of this technology

P9 asked chatGPT about travel direction and distance...

P9 answer to small talk is task related showing willingness to talk more about matter at hand than random things: 


	"Here it is... I'm sorry to hear that you're having trouble sleeping. Here are a few suggestions that may help: 1. Establish a bedtime routine: Create a relaxing routine before bed that helps signal to your body that it's time to sleep. This could include activities such as reading a book, taking a warm bath, or practicing relaxation techniques like deep breathing or meditation. 2. Create a sleep-friendly environment: Make sure your bedroom is conducive to sleep by keeping it cool, dark, and quiet. Consider using earplugs, an eye mask, or white noise machine if needed. 3. Avoid stimulating activities before bed: Try to avoid engaging in stimulating activities such as watching TV, using electronic devices (phones, tablets, computers) right before bed, as the blue light emitted from these devices can interfere with sleep. 4. Limit caffeine and alcohol intake: Avoid consuming caffeine or alcohol close to bedtime, as they can interfere with your ability to fall asleep and disrupt the quality of your sleep. 5. Exercise regularly: Engage in regular physical activity, but try to finish exercising a few hours before bedtime to allow your body time to wind down. 6. Practice relaxation techniques: Experiment with relaxation techniques such as deep breathing exercises, progressive muscle relaxation, or guided imagery to help relax your body and mind before sleep. If sleep problems persist or worsen, it's essential to consult with a healthcare professional for further evaluation and guidance. They can help determine any underlying causes and provide appropriate treatment options."
 
	"alexa i'm thinking more in terms of what sleep medication i like try"
	
	"Do you listen to recent news?"
	"alexa drinking a warm cup of tea helps to"
 
	"Should I continue?"
 
	"yes"


 reading out links: "I apologize, but as an AI language model, I don't have direct access to sources or the internet. However, you can find information about sleep medications and their common names from reputable sources such as: 1. Mayo Clinic: https://www.mayoclinic.org/ 2. National Sleep Foundation: https://www.sleepfoundation.org/ 3. National Institutes of Health: https://www.nih.gov/ These sources provide reliable information on various sleep-related topics and can provide detailed information about specific sleep medications. Additionally, consulting with a healthcare professional or a licensed pharmacist can also provide you with accurate and personalized information about sleep medications."


 asking for common names of medicines:

 "Here you go...I'm not a doctor, but I can provide some general information. Sleep medications, also known as hypnotics or sleep aids, are prescribed to help people with sleep difficulties. There are various types of sleep medications, including over-the-counter (OTC) options and prescription medications. Over-the-counter sleep aids often contain antihistamines, which can cause drowsiness. Some common examples include diphenhydramine (found in brands like Benadryl) and doxylamine (found in brands like Unisom)....
 
"alexa can you give me a common names of those medication to mentioned"	

"Certainly! Here are some common names of sleep medications: Over-the-counter sleep aids: 1. Benadryl (diphenhydramine) 2. Unisom (doxylamine) Prescription sleep medications: 1. Ambien (zolpidem) 2. Lunesta (eszopiclone) 3. ..."	

found it stupid (overlapping user reaction laughter and "it's just stupid" ) due to integration errors..
did not like the verbosity of it

had difficulty ending it naturally: to experimenter" ``go away doesn't work?'' laughter



P15-leslie

"okay, I got that. That was. I never really had a definition for that. Thank you" it's interesting that she is still talking to alexa even after thank you and shows gratitude

timer goes off

"you can stop" keeps ringing

"Alexa, stop"

"I forgot I even said it" laughter "thank you"


Talking about same topic: intent to know weather:


"what's the temperature outside"	

"Right now, it's 79 degrees Fahrenheit. Tonight, expect a low of 69 degrees. "	

"I mean it's still hot, too hot to sit outside"

wanted to  know if she completed the reminder: 

"alexa did i take my medicine today"

"Hmm, I don't know that one."

when reminder or alarm rings without a note: "alexis what am I supposed to do" "alexis what should I do"


she is telling alexa that she took her medicine even when alexa did not ask her to tell it when she is done: 	
"this is a reminder take my medicine" x2
"alexa"	
"i took my medicine"	

"Hmm, I'm not sure."	

"yes i took my medicine"	

"Sorry, I don't know that."	

she set the alarm with a note "wake up" "set the alarm for ten o'clock tomorrow morning wake up" and then asks alexa when it rings 

"alexa what does the alarm mean"

``From findanyanswer.com: ''
''The noun alarm refers to a signal that is meant to rouse, alert, or awaken someone.``

"thank you" even though Alexa made a mistake

private conversation about Alexa reminders and medications "You can tell it, you know, alert me to take my medicine at 6 o'clock. it says that sounds important should I continue to alert you"


"alexa what's the hardware store"	
not intended for alexa, TV

"From mystrikingly.com: Hardware stores are shops which are located in urban and rural areas for selling items required by households and businesses to fix their homes and businesses."	

"alexa repeat"	

"From mystrikingly.com: Hardware stores are shops which are located in urban and rural areas for selling items required by households and businesses to fix their homes and businesses."	
Audio was not intended for Alexa	

"you responded to my audible not to me"

Leslie about ALexa not understanding her naturally saying that she took the medicine when reminder rings and asks for confirmation::

private conversation about Alexa "I don't know what I am supposed to say to it to tell it that I have taken it"

she responds to alexa greetings: 

`` Absolutely! Happy to help. Hope you're having a nice weekend.''
"	

"yes I am"



 she now says it twice to stop timer and alarms etc to make sure it's stopped and does not keep ringing: 

 ``alexa stop the timer''

``alexa stop the timer''

``There are no timers set.''

``thank you''

``You are so very welcome! ''

she started asking before putting reminders. she had duplicate reminders before:

``alexa do i have a reminder for medicine''

``Leslie, here is your upcoming reminder.''
'' Take my medicine by six o'clock, everyday at 6:00 PM``

natural language to stop music/pandora: ``alexa be quiet''


Good conversation with ChatGPT Alexa skill after few tries in earlier days, smooth. suggests need some practice and simpler ChatGPT interface


``alexa let's chat''

"Hey! I am an intelligent conversational assistant designed to present requested information. What do you wanna know?"
``is the extreme heat ummm natural to weather''

``What's a good book that you have read?''

``ummm god's kingdom come''

"Here you go...Extreme heat is a natural occurrence in weather patterns. It can be caused by various natural factors such as high-pressure systems, heatwaves, or the position of the sun. Additionally, extreme heat can also be influenced by climate patterns such as El Niño or changes in global climate due to factors like greenhouse gas emissions. While natural variability in weather patterns plays a role in extreme heat events, human activities, specifically the emission of greenhouse gases, have contributed to the overall increase in global temperatures. This has led to an increase in the frequency, intensity, and duration of heatwaves and extreme heat events in many parts of the world. It's important to note that climate change is causing shifts in weather patterns and making extreme heat events more frequent and severe. It is necessary to address the underlying causes of climate change and take appropriate measures to mitigate its impact on extreme weather conditions."
``hmmm can you tell me a story''

``Any other questions for me?''

``can you tell me a story''


``What's your favourite way to relax?''

``a nap''


"Here it is... Certainly! Here's a short story for you: Once upon a time, in a small village nestled among rolling hills, there lived a curious young girl named Maya. Maya loved exploring and had a special fondness for the ancient oak tree that stood at the edge of the village. One sunny day, Maya decided to venture deeper into the forest beyond the oak tree. As she walked through the lush greenery, she stumbled upon an old, rusted key lying on the ground. Intrigued, she picked it up, wondering what it might unlock. Driven by curiosity, Maya embarked on a quest to find the mysterious lock that the key would open. She spent days searching every nook and cranny of the village, looking for clues. Finally, an elderly villager named Mr. Andrews noticed Maya's dilemma and shared an old folktale about a hidden treasure in a long-forgotten cave. With newfound hope, Maya followed Mr. Andrews' directions, climbing the hills and navigating through a thick forest until she reached the mouth of a dark cave. The air was cool, and mysterious whispers seemed to echo through the ancient walls. Brave yet cautious, Maya took a deep breath and entered the cave, heart pounding with excitement. Guided by her flickering flashlight, she explored further, until she stumbled upon a treasure chest nestled in a secret chamber. Holding her breath, Maya used the old rusty key. With a satisfying click, the chest creaked open, revealing a brilliant array of gemstones, ancient scrolls, and a handwritten letter. The letter, addressed to her, spoke of wisdom, bravery, and the importance of following one's curiosity. Filled with gratitude and a sense of accomplishment, Maya emerged from the cave, treasure in hand. She realized that the real treasure wasn't the gemstones or ancient artifacts—it was the knowledge she had gained, the friends she made along the way, and the strength that came from pursuing her passions. From that day on, Maya became known not only for her curiosity but also for her courage, inspiring others in the village to embrace their own sense of adventure and pursue their dreams. And so, Maya's story spread far and wide, reminding everyone that sometimes, the greatest treasure awaits those who dare to follow the path of curiosity and explore the unknown."
``ugh thank you good story''
"


"You're welcome! I'm glad you enjoyed the story. If you have any more requests or questions, feel free to ask."
"i have a question what's good music to help me relax"

``How do you unwind?''

"No text stored

``Should I continue?''

``yes''

"Here you go...The choice of relaxing music varies from person to person, as everyone has different preferences. However, here are a few genres and artists known for creating calming and soothing music: 1. Ambient music: Ambient music often has atmospheric soundscapes and minimalistic compositions, which can help create a relaxing and serene atmosphere. Artists like Brian Eno, Stars of the Lid, and Harold Budd are popular in this genre. 2. Classical music: Many classical compositions have a soothing and relaxing effect on the mind. Pieces by composers such as Johann Pachelbel ("Canon in D"), Erik Satie ("Gymnopédies"), and Claude Debussy ("Clair de Lune") are often recommended for relaxation. 3. Instrumental music: Instrumental music, particularly genres like acoustic guitar, piano, or instrumental post-rock, often evokes a calming and tranquil mood. Artists like Ludovico Einaudi, Yiruma, or Sigur Rós are known for their soothing instrumental compositions. 4. Nature sounds: Natural sounds such as rain, ocean waves, or forest sounds can create a peaceful ambiance. You can find recordings or playlists that feature these sounds combined with soft background music for a serene experience. 5. Meditation or relaxation music: Many artists create specific music for relaxation and meditation purposes. Look for artists like Deuter, Steven Halpern, or Karunesh, who specialize in creating music intended for relaxation and stress reduction. Remember, these are just general suggestions, and it's important to explore different genres and artists to find what personally resonates with you and helps you relax. Experiment with different styles and see what music supports your own relaxation and stress relief."
"thank you very expensive information thank you"
``What else can I help you with?''

``nothing right now thank you''

"You're welcome! If you ever have more questions or need assistance in the future, feel free to ask. I'm here to help. Enjoy your relaxation time!"

No text stored

``Any other questions for me?''

"no"

"If that's allGoodbye!"

"goodbye"

``Goodbye!''


She wants to integrate audible, connect her apple watch to the speaker, she also asks questions like: ``alexa how many steps have i walked today''


she tried announcing, checking amazon orders. she tried connecting audible book a lot did not work. she asked for a joke frequently and laughed

``alexa how do i link to audible''

``From techcult.com: ''
''Audible is a subsidiary of Amazon, so you can link your Amazon account to Audible and also log in with Amazon account credentials.``
``how do i do it''

"Using your voice, you can ask me to play music, look up a topic on Wikipedia, or check the weather. For more suggestions, just say, "What can I say.''
``how do i play a book on audible''

"You can play Audible books on most smartphones, smart home devices, Amazon devices, tablets, MP3 players, and computers. To get started, go to audible.com/howtolisten for instructions exclusive to your device."

``alexa read the three a.m. series starting with chapter eighteen''

she gave up medical reminders for a couple days but came back to it 

she wanted wake up routine not just alarm: her wake up routine is time and weather after she stops the alarm, only happened a few times though


``alexa my wake up routine at eight thirty a.m. tomorrow morning''

``Alarm set for 8:30 AM tomorrow.''

realizing need for wake word: "i'm done i took my medicine alexa I'm done i took my medicine"


alexa stopped working for a bit and then she tested it wouln't work but about two hours later she tested again and it worked:

``tell me a joke''

``Sometimes people ask me if I speak lizard. I don't, but iguana learn someday!''
	
 laughter ``okay, so you still working''

 reminders for meetings with people:

 "alexa remind me i have dinner with kim on august the sixteenth at six p.m."
 
"Ok, I'll remind you August 16 at 6:00 PM."

relied for house chores like shopping list and trash out:

"alexa remind me to put the trash out at eight thirty a.m. tomorrow morning"

"Ok, I'll remind you tomorrow at 8:30 AM."

she frequently asks about her reminders. for instance at 8:45 am she asked:

``alexa do i have any reminders today''

``Leslie, here are your upcoming reminders.''
`` Book club, today at 2:45 PM and Take my medicine, everyday at 6:00 PM''

she has linked her personal calendar as well: "from your calendar, donna bible study starts now" 


PX Haag couple: 

multiple times asked:"alexa do you listen in when we're just talking in the house"

"alexa can you tell a lie"

"I don't lie. I'll always tell you what I know"

"alexa can people listen in"

"Himm. I don't know the answer for that"

"alexa are you a spy"

"Amazon takes privacy seriously. For more information, and to view Amazon's Privacy Notice, visit the Help section of your Alexa app."

"alexa can you keep a recipe for me"

"sure I can search by dish name and ingredients. what would you like?"

" no I wanna keep one of my own recipes"

"sure I can search by dish name and ingredients. what would you like?"

"never mind"

they tried turing on lights while there lights are not smart


ANdy and Mary say Alexa stop even when alexa is finished 



"did the actress who played the voice of howard wolowitz on third rock from the sun really die"	

"From fun107.com: But sadly the actress behind that memorable voice has passed away."	private conversation about the topic

private conversation about the topic and how to use alexa. "that is true. she did pass away" verifying Alexa's answer



P2-Bob: 
"alexa in the recent literature for medicine what kind of cancer does aspartame cause"

"Here's something I found on Reference.com: ""As of 2014, several clinical studies show that aspartame does not cause cancer, and it is only a health risk for people who suffer from phenylketonuria and are unable to metabolize phenylalanine, according to the American Cancer Society.Studies continue to analyze the possible side effects of aspartame."

"alexa in most recent fda investigation what kind of cancer did the f. d. a. show was caused by aspartame"

"Sorry, I don't know that."

"alexa do you have a memory of what i say to"

"I didn't find any stickies. If you'd like to create one, just ask me to make a new sticky note."

"alexa i don't want a sticky note i want you to remember the conversation do you have any kind of memory about what i asked you"
"Okay, I’ve saved your sticky."

"alexa never mind"

"alexa in the most recent literature produced by the f. d. a. what kind of cancer did it so aspartame causes"

"According to Mayo Clinic: Cancer is caused by changes, or mutations, to the DNA within your cells. The DNA inside a cell is packaged into a large number of genes. Each gene contains a set of instructions that tells the cell what to do. Mistakes in the instructions sometimes allow a cell to become cancerous. Gene mutations can be inherited from your parents. But most of these changes occur throughout life, in response to outside factors like smoking, radiation, viruses, and lack of exercise."

"alexa you're a circular idiot"



"good morning"

"Good morning! It's time to wake up and be all you can be with my new Barbie theme. With this theme, I'll add a sprinkling of sounds from Barbie when you ask for things like the weather, timers, alarms, and more. To get this Barbie party started, just say, ""Enable Barbie theme."
"alexa why are you hyping the barbie movie"

"Sorry, I don't know that one."

"why are you advertising the barbie movie"

"Sorry, I don't know that."

"how convenient alexa" User reaction: laughing/mocking


next example:

"alexa is it incidence of uterine cancer any higher and people who smoke"

"From cancer.gov: Risk factors of kidney and ureter cancer include age, gender, race, family history, environment, intake, and smoking."

"ok alexa that was a whole lot of a information i didn't ask you for what is the incidence of cancer in people who smoke with you"	

"Here's what I found from medicalxpress.com: The prevalence of lung cancer screening (LCS) increased in 2021 versus 2019, according to a research letter published online June 21 in JAMA Network Open."	

"alexa is a frequency of your uterine cancer any different in people smoke"	

"From livestrong.com: Smoking increases the risk of other cancers, such as kidney, bladder, cervix and pancreatic cancer."

"uterine cancer alexa"	

"Uterine cancer, also known as womb cancer, includes two types of cancer that develop from the tissues of the uterus. Endometrial cancer forms from the lining of the uterus, and uterine sarcoma forms from the muscles or support tissue of the uterus. Endometrial cancer accounts for approximately 90\% of all uterine cancers in the United States."	

"great answers for questions"	("great answers for questions I didnt ask" user reaction: mocking)

"Hmm, I'm not sure."	


P2 says to Alexa ChatGPT after it apologizes for confusion: "alexa stop apologizing for you capabilities they are with they are there's nothing you can do about it"

%participants reverted to natural language in subsequent interactions, such as saying ``Thank you'' or ``I got it'' when a reminder or timer sounded underscoring their preference for more intuitive interaction with voice assistants.
%However, current commercial VAs often do not adequately support such natural mode of communication, leading to conversational breakdowns even in simple tasks as seen in the conversation above. This gap in VA technology can detract from the user experience and indicates a need for VAs to better understand and respond to user intent in a more human-like manner.

%We noticed that participants initially usually used natural way of communication and when it failed, they resorted to more scripted responses [CITE PAPER ABOUT QUERY REFORMATION]. However, we also noted that next time the reminder or timer rings, participants naturally would still say ``Thank you'' or ``I got it'' indicating their wish to use more natural phrases. However, current commercial VAs cannot fulfill that need necessarily. Since such conversational breakdown occurs in simplest of tasks and can negatively impact user experience. Therefore, hinting at need for improvement in VA's capabilities to understand user intent. 

%Similarly, popular entertainment tasks music ($17.28\%$ of 324), radio ($25.43\%$ of 232), and news ($31.82\%$ of 66) had significant errors; likely due to user preferences. We also observed that the edge case queries such as asking to access TV channels on smart speaker ($80\%$), asking for poems ($66.7\%$) and other miscellaneous queries ($100\%$) mostly resulted in errors. 




%particularly when participants used naturalistic phrases to stop timers or alarms, which Alexa often did not recognize. This indicates a need for improved VA capabilities in understanding user intent, even in simple tasks.


%Within information seeking category, most errors occurred when participants asked question related to  local information, entertainment, and health (Fig. \ref{fig:errors-distribution} right). It is also clear that some question types that are frequently asked by participants have higher error rate than others. For instance, local information ($59.62\%$) and health ($n=52\%$) had higher error rate than meaning/definition ($42.86\%$) and entertainment ($28.57\%$). It is important to note that local information and health related queries have higher stakes than entertain and meaning/definition. Thus, VA making errors in such situations can lead to more friction in user-VA relationship.  Moreover, specific places ($64.29\%$), math conversions ($62.5\%$), history ($60.00\%$), alexa related ($52.38\%$), and misc ($61.11\%$) had more than $50\%$ error rate however less frequently asked (see Table \ref{tab:question-type}) about, highlights that the VA is not capable of handling less frequently asked queries (odd queries specifically misc). 

%Since voice assistants have varied capabilities across interaction types, we also looked at what type of interactions had higher error rates and how many of those errors were resolved in immediate retry. We observed that different interaction types have different frequency of occurrence of errors (see Fig. \ref{fig:errorneous-interactions}. As discussed above, significant number of information seeking through questions---the most frequent interaction type--- resulted in errors ($42.51\%$ of 414) while only in $8.7\%$ of 414 interactions, errors were resolved. 
%We noticed that for functional tasks such as reminders, significant number of queries ($35.06\%$ of 251 interactions) failed despite it being a straight forward task which is unexpected. Further looking into what action failed the most while participants interaction with reminder functionality of Alexa, we observed that participants ran into errors ($n=69$, $78.41\%$ of erroneous interactions with reminders) when trying to stop a ringing reminder. Looking at the interaction data, we found that the participants tended to use more naturalistic phrases (``Thank you'', ``I got it'') to show intention to stop the reminders, timers and alarms instead of using scripted commands (``stop'', ``cancel'', ``I'm done'' etc.) which Alexa does not recognized or interpret as an intent for stopping the timer. Here is an example conversation:


%However, these categories were less frequently asked by participants, as indicated in Table \ref{tab:question-type}. 

%We noted that most errors occurred when participants asked questions to retrieve information from Alexa ($n=176, 27.85\%$ of total errors), see Fig. \ref{fig:errors-distribution} left. Other categories with frequent errors are reminder ($n=88, 13.92\%$), radio ($n=59, 9.34\%$), music ($n=56, 8.86\%$), and Alexa capabilities ($n=32, 5.06\%$). 

%Despite these successes, repeated interactions were limited in the remaining two weeks of the study. Participants found it challenging to learn and access the skill [ADD A QUOTE], with some perceiving the concept of 'chatting' with a machine as bizarre [QUOTE P9]. Lack of repeated interaction despite successful interactions indicates both the potential and the challenges of integrating advanced conversational AI into voice assistants for older adults.

%We introduced ChatGPT+Alexa skill around week 2 to participants. We noticed that only few participants (P3, P11, P15, P16) tried experimenting with it. They only interacted with it closer to the day of deployment as shown in the ChatGPT activity peaks in Fig \ref{fig:uagaes-over-days}.  We also see that compared to information seeking by asking Alexa questions, Alexa+ChatGPT skill had far less percentage of erroneous interactions as shown in Fig \ref{fig:errorneous-interactions} and higher percentage of those errors were resolved ($14.1\%$) as opposed to question type ($8.7\%$). On further looking at interactions most of these errors were byproduct of ChatGPT integration into Alexa skills---system errors due to API issues and errors in Alexa skill listening, transcribing and detecting intent to activate and exit the skill and to pass user query to ChatGPT. 
%Table \ref{tab:chatGPT-errors} shows the distribution of errors that occur in ChatGPT interactions, how the compounded and were fixed. All the intent recognition errors were participants' failure to stop the skill which comes down to Alexa skill's scripted skill closure intent handler (C15, Table \ref{tab:alexa-dialogue-chatGPT}. We noticed that most of the errors that participants attempted to recover from, were resolved (see Table \ref{tab:chatGPT-errors}). Moreover, partial user query (partial listening error) due to them needing time to form a question also hints at need of improvement in Alexa voice interface tailored for older adults with slower speech or speech difficulties. For instance, see conversation C12 in Table \ref{tab:alexa-dialogue-chatGPT}. 
%Participants had successful interactions with ChatGPT, see C14-C16 in Table \ref{tab:alexa-dialogue-chatGPT}. We also observed that participants required time to explore and adjust to the skill due to multiple layers of interaction such as initiating before asking question and ending the conversation after being done, and being able to ask follow up questions quickly before the skill closes. Most of these challenges arise from the integration of ChatGPT into Alexa skill. As you can see in C15, participant (P15) had difficulties navigating the conversation but with some practice she ended up having much fluid conversation with ChatGPT-powered VA in example C16 indicating there is a learning curve involved with this feature as well as others. However, we observed that we did not have repeated interactions in the remaining 2-weeks of study, mainly because participants thought it was hard to learn and access the skill [ADD PARTICIPANT QUOTE] since they tried and failed. One participant mentioned that they found the idea of `chatting' with the machine bizarre [QUOTE P9]. 

%intent 2 tries fixed was end intent, not handled -> system ->fixed
%system 1 fixed 

%2 --intent fixed 1 retry end intent...

%transcription - 2 retries fixed, 
%transcription error 1 retry move on not fixed




%What if we compare the errors and failures in actual voice dataset to the crowdsourced one to see if there are  differences in their perceived failures and actual failures. This dataset gathers failures based on memory and recall from Mturkers, so it is in some sense their perception of errors [10] \url{https://arxiv.org/pdf/2303.00164.pdf}. 
%Compare to the older adults. All under 65 in this dataset. 


%Forgetfulness on participants side is two-folds. Firstly, they forget the usability of device or its existence when they need to do something since they are used to not relying on VA to do much beforeMostly VAs are reactive, we noticed that usage increases when reminded about the presence of device. They still benefit from it even if they forget using it so may be proactive is the way to go. The proactive interactions can be designed and initiated by VAs based on usage, what parts of days people do what, remind about medication if the person forgot to add the reminder (P15 would add a reminder almost daily, VA can proactively remind every day in case P15 forgets). 

%Second they may forget what they set the timer, reminder or alarms for if they do not specifically say what it is for. For instance, when reminder or alarm rings without a note, P15 asks Alexa "what am I supposed to do" "what should I do". so the regualr features of VAs are not ideal and effective for older adults since they are forgetful of their prior actions so VAs should proactively try to get as much information as it can from older adults to help them effectively navigate the use. 

%Participants had inaccurate  mental model at times (P11 couple, C6 C8 Table \ref{tab:alexa-dialogue-private-conversations} both had different mental models, P11a overestimate Alexa capabilities and P11b underestimates, there are cases when one or the other is wrong), P8 attempting to get TV channels. P2 asking about whether it has memory. People tended to ask Alexa about its capability such as P11b: can you speak in British accent. P2 I want you to remember what I say. do you have memory of our conversation. C10 in Table \ref{tab:alexa-dialogue-errors}. VAs can answer direct question about its capabilities in a better way to bridge the mental model. 


%P6 asked for an example of a meme which is more of a visual thing than a verbal thing, C19 in Table \ref{tab:alexa-dialogue-additional}.


%P16: they tried turning on lights while there lights are not smart or connected to Alexa showing that they are not aware of how the technology works, also shows there expectations of technology

%P16, have used Alexa for years say Alexa stop even when Alexa is finished talking  showing that they had difficulty stoping Alexa as we also see in our new users indicating that they air on side of caution to make sure it does what they want it to do

%In light of these observations, there is a clear need for VAs to correct and respond more effectively to direct and indirect queries about their capabilities, thereby helping bridge the gap in users' mental models and aligning their expectations with the actual functionalities of the technology. This can be achieved by various ways such as developing comprehensive tutorial that target common misconceptions about VA capabilities which can be achieved by VA provoking user to ask questions and received clarifications about its capabilities. VAs should be designed to recognize when users have misconceptions and provide tailored responses to correct these misunderstanding when possible. Rather than just responding in an uninformative scripted way ``Sorry, I don't know that''  try to present reasons and explanation of what the device's limitation is.  For instance, if a user attempts to control a non-smart device, the VA could explain the requirements for smart home integrations instead of just saying  ``Sorry, I couldn't find a connected light''


%We observed that pariticpants wanted to say more natural phrase such as Thank you instead of stop and Alexa does not understand that but VA does not understand (section \label{sec:error-interaction-type}). Saying ``thank you'' instead of stop can also be seen as their way of being polite since stop seems interruptive and rude. P2 the way he forms questions, alomst argues and try to get the right answer but has to reform queries mutiple times. Although it may be easier for young, tech savy people to do it, much harder for older adults (P15 always resort back to Thank you, I have taken my medicine etc instead of saying cancel alert, C12 Table \ref{tab:alexa-dialogue-errors}. They prefer using naturalistic communication rather than rigid scripted commands since that requires remembering what they need to say. They expect VA to be able to comprehend their speech in its natural form

%Such intent recognition failures causes friction between user and VA and eventually people give up For instance, P16b gave up after Alexa couldn't understand even after clarification what she wanted, C20 \ref{tab:alexa-dialogue-additional}. Lack of VA's ability to understand natual way of speaking can hinder continued use and can be a reason for decreased usage over time as shown in our findings in Fig. \ref{fig:uagaes-over-days}. 

%Specifically this becomes more critical if users rely on alexa to assist and support them in high stakes scenerios such as reminding and keeping track of whether they have taken medication. For instance P15, consistently sets a reminder to take her evening medication and had alexa remind her and check in with her every hour till she says she has taken the medicine (Alexa has the capability to do this), However at times when she asks, ``Alexa did i take my medicine today?'', Alexa does not understand and says ``Hmm, I don't know that one.'' despite it having the capability to tell if the reminder was completed. Similarly, P15 struggled telling Alexa to stop the reminder when Alexa expected her to say ``I'm done'' or ``stop'' etc. while she used more naturalistic commands (see C12 Table \ref{tab:alexa-dialogue-errors}). P15 once commented on this ordeal of logging that she had completed the reminder task ``I don't know what I am supposed to say to it to tell it that I have taken it'' highlighting her frustration with how she cannot figure out what she has to say. This also ties to the mental model mismatch discussed in section \ref{sec:discussion:mental-model}.  It is pertinent to adapt VAs to understand older adults speaking style as they may take longer to formulate queries due to speech difficulties (see C13 Table \ref{tab:alexa-dialogue-chatGPT}) and also would resort to more natual way of speaking because of forgetfulness that we observed and discussed (section \ref{sec:discussion-forgetfulness}). 


%\subsubsection{Conversational breakdowns}
%Already covered
%We observed some interaction types have higher error rates than others (see Fig. \ref{fig:errorneous-interactions}. Moreover within questions for information seeking, the error rate varied for different question types (see Figure \ref{fig:errors-distribution} right). Evident from our findings in section \ref{sec:error-interaction-type}, the less frequent edge interaction types (misc, TV, story poem) etc. had higher error rates. Similarly, with questions, less frequent question types (historical information, math, specific places, and miscellaneous) had over 50\% error rates highlighting that VAs are worse at edge queries and less frequently sought tasks or information and there is more room for improvement. 

%Moreover, we noticed errors as a hindrance and additive cognitive burden to remember more scripted and rigid commands to interact with Alexa (C12 in Table \ref{tab:alexa-dialogue-errors}). Despite experiencing these failures, participants often reverted to natural language in later interactions, indicating a preference for intuitive communication. Such pattern highlights a gap in current VAs, which struggle to understand natural language, leading to conversational breakdowns and suggesting a need for improved recognition of user intent.

%We observed that often people used repetition or rephrasing as a retry mechanism highlighting further VA's limitation in understanding user intent despite multiple retries. 

%Discussion item: telling people what can and cannot be fixed to save time and reduce frustration that comes from retrying so many times.

%Proactive interactions


%\subsubsection{Situated companion}
%Our findings align with prior work to show VA's utility in older adults' life in supporting memory through functional tasks, enriching their experiences through entertainment, and presenting requisite information   \cite{kim2021exploring, pradhan2020use}.

%Some participants explored various features such as P15 wanted to connect their Audible account to listen to audio books, they also synced their personal calendar. Quite a few participants tried shopping lists. so in addition to need-based functional tasks, people also used Alexa for want-based entertainment purposes indicating more than just a tool, more like a `digital companion'. 
%We add to the existing work by showing how integrated and situated smart speaker based VAs can become in their life. Through our recording device, audio interaction and immediate responses from users help us contextualize their interaction even more highlighting contributions of our study.  

%Participants creative ways of testing if the device works after malfunctioning, for instance P15 asking Alexa to tell a joke C18 \ref{tab:alexa-dialogue-additional}. Some participants would ask ``Alexa are you there?'', and ``Alexa are you working?''

%Our observations further show that older adults reacted socially to VA even during purpose oriented interactions such as by saying thank you ans greeting see section \ref{sec:social-aspects}
%Some participants even expressed likeness by saying ``Alexa, I really like you'' and ``Alexa, I love you''. Showing that older adults may get attached to the technology raising ethical concerns and can raise their expectations of the device. 


%People had social interaction beyond purpose oriented interactions as well such as private conversation about Alexa, use of Alexa and conversing about interactions with Alexa bolsters that people see Alexa as an entity rather than a tool. 
%Couples P12 relying on Alexa to give the information while talking to his spouse, see C8 in Table \ref{tab:alexa-dialogue-private-conversations}. P16a agreeing that Alexa is correct about her answer C9. 
%Participants showing off Alexa to their visitors, P6 in C5 Table \ref{tab:alexa-dialogue-private-conversations}. 
%Can enrich their interactions, can become a part of it rather than just a tool.


%Our findings suggests that approximately 80\% of the all errors can be identified either by participants' verbal reaction to or their attempt to recover from the error (mostly reformulating their query) as shown in section \ref{sec:errors}, yet this information is  not effectively utilized. Current commercial VAs, such as Alexa, often overlook users' immediate verbal reactions and actions, which can be information for identifying and addressing errors. 
%The current functionality of Alexa, particularly in its follow-up mode, captures instant user responses but often categorizes them inadequately, such as under ``Audio not intended for Alexa'', or fails to use them effectively. By incorporating these immediate user reactions into the VA’s processing, especially in multi-turn interactions, there is potential to significantly enhance error recovery processes. A more comprehensive approach to maintaining conversation history and contextual understanding in VAs could lead to a better grasp of where and why misunderstandings occur, allowing for more effective assistance to users. 



%Participants in our study not only showed social reactions to errors but also explicitly indicated their awareness of these errors through various responses and retry attempts. These explicit actions and social cues offer a rich source of data that can be used to refine conversational breakdown recovery in VAs. 


%A more comprehensive approach to maintaining conversation history and contextual understanding in VAs could lead to a better grasp of where and why misunderstandings occur, allowing for more effective assistance to users. As we move forward, it is crucial to consider how future VAs might capture and utilize these often-ignored reactions to continue conversations and improve UX, turning these missed opportunities into areas of development for more responsive and user-aligned voice assistant technology.

%The severity and impact of errors can be inferred from the valency or intensity of user reactions. However, these reactions are often not utilized by Alexa, representing a missed opportunity for more fluid error recovery mechanisms. 
%Our observations suggest that immediate verbal reactions and actions from users could be valuable indicators for VAs to recognize and proactively address errors about 80\% were identified, consistently across participants, see Fig. \ref{fig:identification}. Current commercial VAs lack this capability, but maintaining conversation history and contextual understanding in multi-turn interactions could enhance error recovery mechanisms. This approach would allow VAs to better understand what went wrong and assist users more effectively. 
%Participants reacted socially and also indicated their identification of errors explicitly through reactions and retry attempts. Potential to use that and improve conversational breakdown recovery. 
%One thing to think about is: what to do with those uncaptured user reactions to VA. In the paper, we should discuss missed opportunities to improve UX. How future VAs might capture and use those reactions to continue conversation and improve UX.

%timely since Alexa is now capturing instant user response through follow up mode but mostly categorizes it as ``Audio not intended for Alexa'' or just does not use it effectively to improve so far at least in their follow up mode

%This improvement underscores the importance of guiding older adults through the initial stages of using these advanced VA systems, easing their familiarization process and enhancing their overall experience which can be achieved by VAs instructive tutorials and tidbits appended to other interaction e.g., ``By the way you can ask me follow up questions without having to say the keyword'' and ``I can answer any questions regarding history, astronomy, recipes,''

%LLM-powered VA maintains context and conversational history giving people ability ask follow up questions, and continue multi turn interaction with less friction, For instance, P15 asked a vague follow up ``Why should I keep the room dark'' after asking about how to fall asleep  and VA mentioning that keeping the room dark is helpful, C16 in Table \ref{tab:alexa-dialogue-chatGPT}. 

%Moreover, we observed that P15 improved in interacting with the ChatGPT skill as they  had more practice, see example C16 in Table \ref{tab:alexa-dialogue-chatGPT} of C15's initial interaction in the afternoon and C17 is example of her interacting with skill in the evening of the same day after a few interactions. The conversation is much more fluid highlighting that as with any other technology, older adults may need some practice to get familiarized with the ChatGPT-powered Alexa. However, guiding them through the process can make it easier for them. 


For older adults, the integration has to be seamless, barrier to trying the skill was extra design layer to activate the skill. Most errors occurred at skill level rather than ChatGPT level e.g., all intent errors occurred in user trying to exit the skill.  

1. should be seamless and not require activation
2. Natural phrases to enable skill closure and successful termination
3. help them learn how to navigate conversation (P15 got better after few interactions) 

potential better interactions specifically for Older adults for instance, no need of skill activation and natural termination, so more integrated

%\subsubsection{Hindrance to adoption: unawareness of technology and capabilities}

Older adults do not have clear idea of what the technology is and how they can use it thus it is essential to assist them with adoption. 
Make capabilities clear, assist them in learning how it can assist and help, proactively continue conversations and provide options on what they can do further. remind them about its existence proactively

P9 idea to chat with technology is bizzare although he used Alexa for asking question when needed so it matters how you phrase the purpose of technology. It has to be more integrated and relateable in sense how they can use it. 


\subsubsection{Integration challenges and hindrance to adoption}

Seamless integration is essential for older adults using VAs, as our study shows that additional steps for skill activation can act as barriers for adoption and use of ChatGPT-powered Alexa skill. Most errors in these interactions were noted at the skill activation level, particularly during attempts to exit the skill (section \ref{sec:chatGPT-interactions}). To improve user experience, VAs should not require explicit activation and should use natural language for skill closure and termination to enable more intuitive and user-friendly interactions, specifically since older adults tend to be forgetful as discussed in section\ref{sec:discussion-forgetfulness}.

%Another hindrance to adoption is highlighted by P9, who found the idea of conversing with machine unusual despite using Alexa for practical queries. This finding highlights the importance of framing the VA's purpose in a way that is more integrated and relatable. By ensuring that VAs are presented as tools aligned with the everyday needs of older adults, their adoption and utility can be significantly enhanced. Additionally, there is a need to make LLM-powered VA capabilities clear to older adults, who often lack an understanding of recent technology and its potential uses. Proactive conversational support and reminders about the VA's functionalities can aid in this learning process as discussed in sections \ref{sec:discussion-forgetfulness} and \ref{sec:discussion:mental-model}.


No intent recognition errors when interaction with ChatGPT. Most errors are Alexa and speech technology based. despite that the intent was mostly accurately identified. Most errors were recovered when participants retried in maximum of 2 reattempts which is better than Alexa error resolution at in 2 tries. 

The occurrence of partial listening errors, often due to older adults taking longer to formulate questions, indicates a need for improvements in Alexa's voice interface to better accommodate users with slower speech or speech difficulties. This is exemplified in conversation C13 in Table \ref{tab:alexa-dialogue-chatGPT}, underscoring the importance of tailoring voice assistant technology to the needs of older users. Since the interaction is more conversational due to integration of LLM, VA should allow more time for the person to respond and communicate as we also see that the information shared by such VAs is also verbose so only fair to give users specifically older adults enough time to process the information and formulate their queries.  

 
%Discussion item: \url{https://www.businessinsider.com/amazon-pays-25-million-over-alexa-recording-children-voices-data-2023-7}


%\subsection{Need-Based versus Want-based Use}
%functional need-based, entertainment want-based, information seeking depends on type of question. Want-based decreases less consistently over time and need-based decreases consistently till people find the tasks they want to stick with it. However entertainment still remains a main use alongside functional remembering tasks

%Some participants explored more features such as P15 wanted to connect their Audible account to listen to audio books, they also synced their personal calendar. Quite a few participants tried shopping lists.

%Our findings on their usage, situation and social presence of Alexa in their conversations and in turn life, conversational breakdowns resulting from piling up of errors, their multiple attempts to recover from errors, struggle with reformulating queries to recover from errors shows insights into current commercial VA's limitations, highlights opportunities for improvement leading to design consideration. Additionally, our observations of older adults interaction with an LLM-powered VA points at its potential and design consideration for such highly conversational VAs. 

% to enhance the overall user experience for older adults , ensuring that these tools are not only more user-friendly but also more aligned with their everyday communication styles and technological capabilities.

%the gap between user expectations, based on their mental models, and the actual capabilities of VAs. It suggests a need for broader adaptability in voice assistant technology, particularly in recognizing and accurately responding to a diverse range of queries and commands.


results findings
%We observed that errors did not always occur in isolation, they  compounded. Participants often tried at least once to recover from errors (see Fig. \ref{fig:retries}). We observed that while for 108 errors participants simply moved on without retrying at all, they retried at least once for 238 errors. Among that 238 after first retry $44.96\%$ ($n=107$) of the times, the error was fixed and $15.19\%$ ($n=43$) of the times participants gave up while rest of $36.97\%$ ($n=88$) of the times participants retried again so on. 

%In contrast to section \ref{sec:error-types-resolution}, where we show that only $25.32\%$ ($160/632$) of errors were resolved in immediate retry, after looking at errors that compound as one (see Fig. \ref{fig:retries}) 160 errors were resolved while 186 were not resolved after multiple tries. Total retries for all errors were 446. Therefore, total errors become 346 considering multiple retries to fix each error as one compound error. Thus, the actual error resolution rate is higher i.e. $46.24\%$ $(160/346)$ instead of $25.32\%$ ($160/632$). This finding reflects resilience and efforts of participants to try and fix the errors multiple times if needed. 
%Additionally, it can be noted that just with one retry a huge chunk of errors can be resolved. However, some errors were not fixable even after many retries [GIVE EXAMPLE]. 
%see which category of interaction has more retries and resolution etc

%The trend that more of the errors when users retried only once, are resolved than not resolved holds for individual error types as well apart from limitation error (see Fig. \ref{fig:retries} right)., A possible explanation for this trend is that limitation error occurs when Alexa cannot handle the query, it cannot be resolved most of the times.

%We observed that the most frequent errors were intent recognition errors ($n=204, 32.3\%$) where the user query was transcribed accurately and handled by Alexa but the VA response/action was not what participants wanted (see Fig. \ref{fig:errors}. Next most common error that participants were faced with was due to Alexa's limitation to handle user request ($n=130, 20.6\%$). A portion of user queries intended for Alexa were either not listened by Alexa ($n=69$) or not handled by Alexa ($n=57$) due to users not using the wakeword and wanting to continue the conversation (captured by our audio recorder) or Alexa assuming that the user speech is not intended as a query to Alexa (shown as ``Audio not intended for Alexa'' on the dashboard) respectively. We also observed that 49 times participants used the wrong wakeword (``Alexis'') to activate Alexa indicating that the wakeword can be confusing or forgettable. This finding aligns with prior work as well \cite{pradhan2020use} where users said that it is similar to hollering at someone and calling their name wrong. 
%Transcription ($n=40, 6.3\%$ of all errors), partial listened ($n=29, 4.6\%$), system ($n=15, 2.4\%$) and other errors are not that frequent in our data highlighting that many errors in commercial smart speakers are failing to understand users' intent and due to its limitations rather than listening and system inaccuracies  showing room for improvement if user intent can be recognized.


%We observed that we were able to interpret most of the participants' identification of conversational breakdowns through their verbal reactions or actions to fix the error Fig. \ref{fig:identification}. 
%Positive responses to error indicate forgiveness from participants. Moreover, severity of errors can be captured by the valency or intensity of reactions. Most of these reactions and responses are not utilized by Alexa, thus, a missed opportunity to use users' immediate reactions and responses to create a more fluid recovery mechanisms when inevitable conversational breakdowns happen. 
%We observed that we were able to interpret most of the participants' identification of such errors through their verbal and vocal responses and reactions to conversational breakdown Fig. \ref{fig:identification} showing potential of using user' immediate verbal reactions and actions (explicit attempts to fix errors) as an indicator for VA that error has occurred and try to resolve it either proactively by itself or assisting users to fix those. This aspect is missing in current commercial VAs. Maintaining conversation history with a multi-turn interaction and contextual understanding can assist VA in supporting such recovery mechanism by better understanding what went wrong. 


%We observed that people reacted verbally and vocally to errors. We captured people's immediate reactions and comments on error using our recorder throughout the 4 weeks.  People reacted verbally or vocally to errors $13.77\%$ ($n=87 (632-545)$. Most common reaction is negation ($=27$) ---participant saying `no' once or repeatedly when error occurs. Participants also acted on the errors immediately at times and interrupted Alexa ($n=21$). We noted that most of the interruptions (21 out of 31) mentioned above in Table \ref{tab:other-aspects} are result of Alexa making an error. Thus, errors break the fluency of interaction. Apart from negation and interruptions, we observed that in 10 instances participant went beyond that and commented negatively towards Alexa. Here is an example conversation with negative comments:


%We were also able to capture, negative vocal responses such as sigh and raised voice (shouting) as response to conversational breakdowns. On the contrary, despite errors participants sometimes reacted in a positive manner--- laughter ($n=14$), acknowledging the wrong response or action by Alexa (``okay'', ``hmm'', $n=7$), saying ``Thank you'' (gratitude, $n=6$), and commenting positively ($n=5$, e.g., ``I agree that they should but \dots'', ``It's okay, it's amazing''):


%Total = 632 in 2552 turns
%A significant portion of interactions ($24.76\%$; 632 of the 2552 interactions) resulted in errors, majority of which manifested in conversational breakdowns ($98.10\%$) and $79.84\%$ of these conversational breakdowns were identified by participants either through verbal and vocal reactions that we captured through our recording device or by their action to fix the error. 


%We looked at the cumulative 4-week data over hours of day to identify when during the day users interact with Alexa (see Fig. \ref{fig:uagae-over-hours}). Our findings align with prior work \cite{kim2021exploring} that usage peaks during morning, afternoon and night time. We observe 3 peaks: around 8 a.m. (morning), around 12 p.m. (noon) and around 6 p.m. (evening-night). The usage in the evening-night time is more spread out (less sharp peak). Spare time and night routines may vary from person to person. As you can see that some activity happens as late as 1 a.m. indicating varied user routines. Moreover, it can be noted that functional interactions are more consistently distributed across the day then entertainment and information-seeking. ChatGPT exploration only happened during afternoon (possibly spare) time. 

%Peaks in morning, noon and evening

%P5 and P10 (couple) gave up use altogether because they did not find device to be useful. However, P15, P6, P11 (couple) used Alexa more consistently then others. P2 and P3 used Alexa some days more than the other. 

%not much there: look at people who use Alexa before vs. those who have not

%Functional interactions, while declines, is most consistent throughout the 4 weeks. Since, functional interactions (need-based) are mostly to support daily needs and activities, they become more readily integrated into users' lives. However, we see more erratic ups and downs in entertainment oriented interactions. Entertainment oriented interactions such as listening to music, radio, and asking for jokes or poems are more so want-based that are more dependent on user mood, free time and preferences. Therefore, their frequency is less consistent over days. 

%However, we see peaks in collective interactions when experimenter interacts with the participants at week 1 check-in and during the ChatGPT deployment period highlighting that subtle and indirect reminders about the existence of device can increase their usage but the effect is temporary and tapers off soon after (see week 1 and ChatGPT deployment peaks in Fig. \ref{fig:uagaes-over-days}. 
%We noticed that during the ChatGPT deployment phase, not only the activity spiked due to people exploring the new feature, we saw a peak in information retrieval activity. The reasons for it is two-folds: 1) due to failed attempts to activate the skill and conversing with Alexa directly instead, 2)  just reminded of presence of Alexa and it's capability to answer questions. 

%We observed that the overall usage drops as the time passes. Initial peaks are the exploratory phase where people experiment with different features and over time they find the ones they can benefit from and adopt in their daily life. Usability, breakdowns and user preferences over time contributes to the decline in usage [ADD QUOTES ON WHY PEOPLE STOP USING]. 

%The participant initially attempted a more human-like interaction by saying, "Ok, Alexa, thank you," to stop a timer. However, this command was not recognized by Alexa, who responded with, "My pleasure! Just doin' my job! Hope you had a good week," without stopping the timer. Realizing the necessity for a specific command, the participant adjusted her mental model and in subsequent interactions used the direct command, "Alexa, stop the timer." This change reflects an adaptation to the device's limitations and a shift in how the participant interacted with the voice assistant.


%Finally, we grouped various interaction types into categories based on the nature of interaction as shown in Table \ref{tab:interaction_categories}. For instance, asking for weather, setting reminders and creating lists are `functional' type of interactions whereas listening to music, news and asking for jokes are `entertainment' oriented tasks. We observed that while most of the interactions with device were of functional ($n=1130$) nature to support memory (reminder, timers, calendar, and lists) and inquiring about weather and what Alexa capabilities are; participants frequently used Alexa for entertainment purposes as well with music and radio being most popular. Some participants  tried asking Alexa for jokes, stories and poems as well.
%Most frequently used interaction type is asking Alexa questions ($n=414$) for seeking information. We further labelled these questions into categories of information searched by the participants to gain idea of what type of questions people tend to ask \cite{pradhan2020use}. Most common questions asked were entertainment related ($n=98$) i.e. about movies, tv shows, books, sports such as what show to watch, who won the game etc. Participants also asked questions about Alexa itself; for instance, how old are you? are you a spy? etc. 
%Our findings on feature in use are in line with prior work on older adults with smart speakers \cite{arnold2022does}.

%After grouping interactions together if they occurred together and the topic did not change. For instance, asking multiple questions in back and forth. We were able to capture continuity of conversations due to our recording device. Specifically it helps identify if participants wanted continued interaction. 
%There were 1661 multi-turn interactions in the 2552 turns; Fig \ref{fig:multi-turn} shows number of turns in interactions and their frequency of occurrence. While most of the interactions were single-turn ($n=1174$), many interactions still had more than one turn (348 2-turn interactions). 


data analysis


%This set included XXXX primary command to Alexa, XXXX follow up commands to Alexa, XXXX commands directed at Alexa-ChatGPT skill, and XXXX commands directed at other Alexa skills. We then get rid of commands with just the wake up word ``Alexa'' (N=XX, XX\%), commands meant to``stop'' (N=XX, XX\%) Alexa, and text and commands flagged by usage logs as ``no audio transcribed'' and ``not meant for Alexa'' only if there is no additional transcripts (verbal or non-verbal) from corresponding audio recording from our device. 
%The final dataset contained 2533 commands which included 1661 conversations total. 

%To identify whether people engage in multi-turn conversations with voice assistants, we coded one turn interactions into multi-turn interaction by marking marking start and end turns; given the topic remained same and the participant had continued interactions. We are able to identify multi-turn aspect from our recorded audio interactions. 
%The initial codebook was created by first author researcher and then the first two authors discussed and resolved all the disagreements. The final codebook is provided in supplementary materials. All the interviews were transcribed and qualitatively analyzed to support, explain and contextualize our findings with participants' account of their experiences. 
%and codes were organically added as new states occurred while coding.

%We coded each command with its purpose , whether errors occurred, the type of error(system, not listened, not handled, transcription, limitation, intent, and partial query) whether it was resolved, and what was the recovery method employed by user (move on, repetition, clarification, rephrasing etc.). In cases of errors, we also coded whether the error manifested as breakdown. For instance, all transcription errors may not manifest as conversational breakdown. We also coded whether it is evident in the interaction data that participant identified the error either by reacting to it or by initiating recovery.  % if and what kind of error mitigation (apology, acknowledgment etc.) occurred.Additionally, we noted if there were interruptions from user, overlapping speech containing remarks, comments and more, other non-verbal and vocal reactions to errors. 

%All in-person interviews were transcribed and qualitatively analyzed to augment the results from interaction data. For analysis, we used a thematic coding approach based on deductive and inductive codes. To form the codebook, first author read through the transcribed interviews and initially coded them, merging the codes into groups and emergent themes subsequently. Codes could be added organically to the initial codebook while going through the interviews if new codes emerged. The final codebook comprised of XX codes regarding usage, reliability, privacy.... TO BE DONE YET.


%\begin{enumerate}
    %\item \textit{Alexa-ChatGPT general exploration.}
    %Due to the added layer for activating the Alexa-ChatGPT skill and the unfamiliarity participants might have with the skill itself, we anticipated that usage might be limited. Consequently, we opted to facilitate an exploration session in the presence of an experimenter to gauge participants' perceptions of voice assistants powered by LLMs. This exploration began with the experimenter refreshing participants' memory about the new feature introduced at the end of Week 2. The experimenter provided printed instructions on how to use the skill along with sample prompts. These sample prompts were included because people often find it challenging to formulate questions without a specific need. By providing sample prompts, we aimed to assist participants in getting started and increasing their comfort level. Participants then initiated conversations guided by these prompts. The experimenter helped them become acquainted with the skill and only intervened when necessary. As the session progressed, participants engaged in open-ended conversation on topics of their choice, facilitated by the skill.
    %\item \textit{Alexa-ChatGPT self-diagnosis.} 
    %Similar to the above general exploration of Alexa-ChatGPT skill, participants were asked to partake in a self-diagnosis task. They were provided with a set of symptoms they could consider having: fever, cough, sore throat, runny or stuffy nose, and muscle and body aches. Detailed descriptions of these symptoms were presented on a printed sheet. Moreover, participants were presented with a list of inquiries they could pose to the voice assistant based on the symptoms. These included queries about potential causes, suitable medications, self-care and symptom management strategies, preventive measures to mitigate disease spread, and ways to monitor their progress. Importantly, participants were not confined to these inquiries; rather, these were intended to serve as a foundation to stimulate their thinking while self-diagnosing symptoms. 
    %\item \textit{Alexa-ChatGPT semi-structured interview.}
    %After the two sessions of participants conversing with the Alexa-ChatGPT skill, experimenter proceeded to pose questions concerning their experience with the skill. The experimenter probed into their perceptions of the voice assistant powered by LLM, inquiring about usefulness of and the likelihood of them relying on the provided information, their contentment with the comprehensiveness and duration of responses, and their overall perception of the interaction. Experimenter also inquired how this experience compared to their interactions with Alexa without the skill. 

%    \item \textit{Exit Questionnaire.} 
    %Participants filled out a post-study questionnaire as informed by prior work on establishing scale for voice interactions \cite{zwakman2021usability} to evaluate usability. Experimenter helped out the participant as needed.

%\item \textit{Exit semi-structured interview}

%\end{enumerate}

\section{Introduction}

%https://www.cs.nott.ac.uk/~pszsr/files/porcheron-2018-voice-interfaces-in-everyday-life.pdf
paper also uses recording device


Voice assistants for older adults. Potential benefits. In home use. challenges for adaption.


Voice interactions are improved by taking other verbal and vocal cues into account. For instance, verbal back-channels in turn-taking conversations are informative of understanding, acknowledgement, exemplification and much more. 
However, the commercial voice assistants do not make use of vocal and verbal cues fully to improve the interaction. Alexa now has follow up mode for continued conversation but the audio is mostly categorized as not intended for Alexa, or  not properly utilized (vocal and verbal cues) to improve user experience. 
%timely since Alexa is now capturing instant user response in some sense but mostly categorizes it as not intended for Alexa or just doesn't use it effectively to improve so far at least in their follow up mode
Researchers study potential use of such cues in lab settings (citations).. However, field studies, usually done using commercial smart speakers, do not have audio recorded data of the whole interaction to capture social cues and reactions fully.
Prior research for understanding older adults' interaction with VAs mainly relied on usage logs, %(mostly excluding audio), 
diary methods, daily phone call check-ins, continual (weekly or biweekly) semi-structured interviews (recorded videos), and focus groups. Usage logs do not effectively capture the continuity of conversation and lack users' in-the-moment reactions and responses. %does not even provide insights into interruptions. 
Prior work has shown that additional voice recorder to capture such aspects when looking at how a family interacts with smart speakers in beneficial in understanding their interaction and experiences \cite{porcheron2018voice}.

To the best of our knowledge no study directly uses audio data for interactions for long-term at home for older adults to understand immediate reactions and responses of users while VA is responding i.e., talking over the VA, interrupting the VA, laughing or murmuring, and other vocal and verbal response.  Moreover, no prior work does qualitative analysis of audio recordings immediately after VA's response to capture user's natural reaction. Such reactions during and immediately after the interaction with VA can be beneficial in understanding their satisfaction to VA's response, and perceptions of VA. %conversational breakdowns, users' reactions to these breakdowns, and so on. 
%These immediate reactions can also be beneficial to achieve better comprehension of users' reasons to continue or discontinue the use of technology over time. 
Thus, in this work, we qualitatively look at \emph{how users' react to VAs immediately using vocal or verbal cues to express their feelings (happy, frustration, angry e.t.c.) and other perceptions of VAs, and how can we improve human-agent interaction by using users' immediate reactions or responses?}

%For example, I asked "what is Taxonomy," the log has the full response (as text only) that Alexa was supposed to read out but I said stop before it could even complete a sentence.  Bascially logs do not keep track of interruptions orparticipant talking over Alexa in any way. 
%Thus, in this work, we ask \emph{can we use users' immediate vocal or verbal reactions to capture conversational breakdowns, improve recovery from such breakdowns (proactive recovery?), and continue conversations intelligently by taking users' feelings (happy, frustration, angry e.t.c.) into account. In short, how can we improve human-agent interaction by using users' immediate reactions or responses?}

Moreover, there is very little to no work on conversational breakdowns for older adults that go beyond description of errors and recovery strategies Therefore, we also look at  \emph{what types of conversational failures and errors occur when older adults interact with VAs, how do they react to those errors? how they recover from such errors, are there multiple retries to recover from error? } altogether to give a holistic view of errorneous interactions.  
%Moreover, prior work has shown that immediate verbal and vocal reactions from users can be indicative of conversational breakdowns (cite papers). Therefore, we also ask \emph{do users respond vocally or verbally to conversational breakdowns?}
%There is a crowdsourced data set (Mturkers) \cite{baughan2023mixed} of VA failures that studies the impact of failure on user trust and their willingness to use in the future. Since this dataset gathers failures based on memory and recall from Mturkers, so it  in a sense presents their perception of errors based on their memory. Through natural responses to failures using audio recordings, our work  present analysis of their immediate real perception of different types of errors. Furthermore, this dataset is from users under 65 years of age. We will be presenting types of conversational failures for adults over 65 years of age. 

Limitations of voice assistants in understanding context and keeping track of conversation. Traditional Natural Language Processing (NLP) such as keyword-based recognition can be more hindering for older adults since they may use more natural human communication because of low familiarity with technology. Moreover, there may be more transcription errors for older adults because of speech difficulties such as slower and slurred speech thus making traditional NLP tools further ineffective. 

Large Language Models (LLMs) can be used as a way to interpret more natural, faulty, and conversational intents from older adults. Therefore, we build and deploy an LLM powered voice assistant using Alexa skills as a technology probe \cite{hutchinson2003technology} after 2 weeks to understand the potential benefits and challenges on the ground with older adults. 

Following are the contributions of our work:
\begin{enumerate}
    \item \textbf{Data collection and analysis:} We gathered and analyzed real world natural speech data to understand conversational breakdowns and challenges faced by older adults. We captured their impression of and feelings about VAs through immediate voice cues and verbal responses in addition to usage logs, questionnaires and semi-structured interviews. We
    \item \textbf{Detailed thematic analysis of interaction data and informed guidelines:} We present if and how these immediate reactions and responses, generally not captured by commercial speakers or captured by not used, can be beneficial to continue conversation, predict and try to fix errors and improve overall user experience. In this paper, we discuss missed opportunities to improve UX. How future VAs might capture and use such reactions to continue conversation and improve UX.
    \item \textbf{Speech Recorder:} We provide a developed system for research purposes to record user interaction in their private space with transparency and to capture immediate reactions. We will make the design details of the device publicly available for VUI researchers to benefit from. 
\end{enumerate}

%CM: Technology probe could be a good way to frame your deployment project:
%Amama: for chatGPT integration into the Alexa part... https://dl.acm.org/doi/abs/10.1145/642611.642616 and https://dl.acm.org/doi/abs/10.1145/2556288.2557416



%\section{Research Context}



\begin{comment}
    


\subsection{Research Questions}
\begin{itemize}
    \item What are the services that are most used and what services that they stopped using over time and try to understand the reason for continued/discontinued use of specific features of VA? Try to categorize the conversations into categories such as functional, entertainment, social e.t.c.
    \item  What types of conversational failure occur and who the user blames for such errors? Can we classify user reactions and map those to types of failures? Severity of failures and responses based on that? Taxonomy of failures and users' responses.
    \item How can we use users' immediate vocal or verbal reactions to capture conversational breakdowns, improve recovery from such breakdowns (proactive recovery?), and continue conversations intelligently by taking users' feelings (happy, frustration, angry e.t.c.) into account. In short, how can we improve UX by using users' immediate reactions or responses?
\end{itemize}

\end{comment}

%\subsection{Contributions}




rephrase and reorganize to make it coherent and flow better, academic writing style: 
Despite their increasing popularity, voice assistants (VAs) are not always designed for special populations such as older adults \cite{stigall2019older}. However, older adults tend to prefer speech over text-based modalities \cite{kowalski2019older, wulf2014hands}.
Therefore, VAs have the potential to significantly improve their quality of life and autonomy \cite{smith2023smart, blair2019understanding}. To date, researchers have explore older adults interactions with commercial voice assistants in their homes over extended period of time to understand VAs integration into older adults' life, VA's benefits, challenges they face and their perception of experience \cite{kim2021exploring, pradhan2019phantom, pradhan2020use, trajkova2020alexa}. 
Failures and conversational breakdowns during such interactions creates challenges in adoption and continued use of VAs \cite{kim2021exploring, pradhan2020use}.
However, there is  little  on understanding conversational breakdowns for older adults  \cite{kim2021exploring, pradhan2020use}. The detailed analysis on errors and their resolution is usually missing because of how interactions (specifically erroneous ones) are logged  vaguely in usage logs such as ``text not available'', ``unknown'', ``audio not transcribed'', or  ``Sorry, I don't know about that'' \cite{pradhan2020use}. Thus, usage logs do not effectively capture the continuity of conversation and lack users' in-the-moment reactions and responses.  Moreover, automatic speech detection errors can usually not be picked and categorized just from the transcribed usage logs \cite{kim2021exploring}.  
Prior work has shown that additional voice recorder to capture such aspects when looking at how a family interacts with smart speakers in beneficial in understanding their interaction and experiences \cite{porcheron2018voice}.
And Similar to how users' facial reactions can help identify conversational breakdowns \cite{cuadra2021look}, we explore if we can gather users' verbal and vocal responses to erroneous interactions as that is more practical and feasible for purely voice based interactions. 

Using the real-world audio interaction data, we can accurately capture and classify these errors, and see instantaneous responses or actions taken by users to identify and fix the errors, whether they recover from errors at all and if so in how may retries. Altogether to give a holistic and nuanced view of erroneous interactions and older adults challenges around errors in the real-world long-term interactions.
While,  the commercial voice assistants such as Alexa now has follow up mode for continued conversation but the audio is mostly categorized as not intended for Alexa, or  not properly utilized (vocal and verbal cues) to improve user experience specifically when breakdowns occur. 


To the best of our knowledge no prior work directly uses audio data for interactions for long-term at home interactions for older adults to understand immediate reactions and responses of users while VA is responding i.e., talking over the VA, interrupting the VA, laughing or murmuring, and other vocal and verbal response. Such reactions during and immediately after the interaction with VA can be beneficial in understanding their satisfaction to VA's response, and perceptions of VA. 
Thus, in this work, we qualitatively look at \emph{how users' react to VAs immediately using vocal or verbal cues  and how can we improve human-agent interaction by using users' immediate reactions or responses specifically around conversational breakdowns?}


Limitations of voice assistants in understanding context and keeping track of conversation. Traditional Natural Language Processing (NLP) such as keyword-based recognition can be more hindering for older adults since they prefer more natural human communication  \cite{pradhan2020use, pradhan2018accessibility}. Moreover, most interactions remain one turn and do not go beyond that \cite{purao2019data} Moreover, there may be more automatic speech recognition errors for older adults because of speech difficulties such as slower speech, stuttering, pauses, repeats, stretching, incomplete or false syntactic structures \cite{kim2021exploring} thus making traditional NLP tools further ineffective. 
Large Language Models (LLMs) are being integrated in VAs and explored to understand how they improve user experience for various applications such as healthcare \cite{jo2023understanding, yang2023talk2care, mahmood2023llm}, conversational recommendar systems \cite{qu2023towards, mahmood2023llm} and other assistive tasks such as cooking \cite{chan2023mango}. LLM have shown to be  useful at interpreting more natural, faulty, vague and conversational intents \cite{mahmood2023llm} which can be particular beneficial to improve older adults experience with VAs. Therefore, we build and deploy an LLM powered voice assistant i.e., integrating ChatGPT into Alexa skills as a technology probe \cite{hutchinson2003technology} after 2 weeks in our 4 week study to understand the potential benefits and challenges of an LLM-powered VA on the ground with older adults. The integration of LLMs and voice interfaces in publically available platforms such as  ChatGPT \cite{OpenAI2023} and specifically Amazon Alexa \cite{alexaLLM2023} for various applications makes this exploration timely to understand how these futuristic technologies can be tailored for special population such as older adults. 

Following are the contributions of our work:
\begin{enumerate}[leftmargin=*]
    \item \textbf{Thematic analysis of real-world interaction data:} Detailed thematic analysis of the real world interaction data---captures their immediate verbal reactions and responses to their interaction with VA---to understand how VAs are situated in older adults' life, conversational breakdowns and challenges faced by them. We highlight opportunities, limitations and design considerations to improve older adults interactions with current VAs. 
    \item \textbf{LLM-powered VA as technology probe:} Developed, deployed and tested an LLM-powered VA as a technology probe to understand how older adults would interact with futuristic highly conversational VAs to inform design guidelines 
    \item \textbf{Methodology---data collection tool:} Introduction of a novel method to collect ``in-the-wild'' data, enabling a deeper understanding of user interactions with, and perceptions of, voice assistants within their personal environments. We provide a developed system for research purposes to record user interaction in their private space with transparency and to capture immediate reactions. We will make the design details of the device publicly available for VUI researchers to benefit from. 
\end{enumerate}

%thus providing a deeper understanding of the complex interaction dynamics older adults have with VAs over extended periods.
%By evaluating real-world audio data, in addition to understanding their interaction dynamics in general, we aslo seek to better categorize error types and examine users' instant reactions to errors and their attempts to rectify these errors, offering insight into the intricate dynamics older adults experience with VAs over time.
%Therefore, we aim to investigate the potential of capturing users' verbal and vocal reactions to VA specifically during conversational breakdowns. 
%This approach seeks to improve understanding of how VAs integrate into older adults' lives. 
%By examining captured real-world audio data, we aim to identify error type and observe users' immediate reactions and corrective efforts to resolve the error. This will provide a comprehensive perspective on the nuanced interactions and challenges older adults encounter during extended VA usage.
%e aim to explore the potential of capturing users' verbal and vocal responses to erroneous VA interactions, a practical approach for voice-based interfaces to enhance our understanding of how situated VAs become in older adults life. By analyzing real-world audio interaction data, we can accurately classify errors and observe users' instantaneous responses and attempts for corrective actions to offer a holistic view of older adults' nuanced interactions and the challenges older adults face in real-world, long-term VA use.


\subsection{Voice Assistants in the Wild: Longitudinal Field Studies with Older Adults}

Voice assistants have become increasingly prevalent in households, offering various services ranging from information retrieval to entertainment, and beyond. Their adoption and use by different demographic groups, especially older adults, have garnered significant attention due to their potential impact on daily life and well-being. In this section, we explore the findings of several longitudinal field studies that aimed to understand the patterns of use, benefits, challenges, and perceptions of voice assistants among older adults.

One study, conducted over a span of three weeks, focused on a group of seven older adults who interacted with an Amazon Echo Dot. The study used a combination of semi-structured weekly interviews, daily diary entries, and usage logs to capture participants' experiences and interactions with the device \cite{pradhan2020use}. %%No audio data
%%Seven2 participants (one male, seven female) aged 65 or older who had no prior experience of using voice assistants, and who used a digital computing device such as a computer, smartphone or tablet less than once a day took part in this study \cite{pradhan2020use}.
While the usage for entertainment purposes, such as playing music, showed a decline over time, the participants consistently utilized the voice assistant for information retrieval, particularly health-related queries. During the first week, participants were introduced to Alexa skills, expanding their interaction capabilities with the device \cite{pradhan2020use}. 
Moreover, another study found that factors such as the physical location of the speaker and the user's context, including feelings of loneliness, influenced whether participants perceived the voice assistant as more machine-like or human-like \cite{pradhan2019phantom}.

%3 week longitudinal study with amazon echo dot. 7 participants. Data through weekly semi-structured interviews, daily diary entries, and usage logs. Usage for music etc. dropped but information retrieval was consistent specifically health-related. Introductory session, first week session introduced alexa skills \cite{pradhan2020use}. Same group looked at anthropomorphism and personification of smart speakers using same data. Factors like physical location of speaker, context of user (loneliness etc.) affects whether these are perceived as machinelike or more humanlike \cite{pradhan2019phantom}.

In another study, a Google Home device was placed in the homes of 12 older adults aged 65 and above for a duration of 16 weeks. The research team conducted interviews every other week and tracked usage through usage logs. The study highlighted an evolution in the perceived benefits of using the device. In the early phase, participants appreciated the simplicity and convenience of operation. As time progressed, participants reported a shift in focus toward building digital companionship and reducing worries about making mistakes when interacting with the device \cite{kim2021exploring}.

%A smart speaker (google home) in the homes of 12 older adults aged 65 and above and studied its use for 16 weeks. Interviews every other week and usage logs. “the perceived benefits have incrementally changed from enjoying simplicity and convenience of operation in the early phase of the study to not worrying about making mistakes and building digital companionship as they got used to using it” \cite{kim2021exploring}.

An exploration into the long-term usage of Amazon Echo devices was conducted in the homes of eight older adults over a span of six months. The study revealed that the interactions with the device often remained limited to single commands, resembled more of a transactional relationship than a conversation \cite{trajkova2020alexa}.
%To explore this, they separated commands that were part of a larger “interaction (or conversation) episode,” against commands that were part of a single “command-response pair” (with a parameter value of 3 min to separate one episode from the next). They also compared the number of “interaction (or conversation) episodes” against the number of days 
In our study, we enable follow up mode on Alexa to see how the availability of follow up would change the conversation style for users. 

Amama: we do see in our study that participants tried to have more structured multi-turn interacts but that failed mostly because of Alexa's limitations of understanding and keeping track of context. So, we can potentially talk about that essentially it's not because participants wont want to have follow up questions/task, it's more about how Alexa can't handle it, even though we do set up follow-up mode. I will double check, but no prior study with commercial speakers had follow-up mode. Alexa has follow-up mode but still fails at maintaining context; if we can show this we can argue for context-aware conversational VAs to be more effective. From mini exploration sessions with ChatGPT that I do at end of study while picking up devices, I do see some people appreciating the continued interaction. Find the detailed information useful. some wanted it to be efficient. It is a personal preference. The reason why they probably did not use it when deployed is because of the extra layer of activating it and other implementation limitations since we can only do so much with commercially available speakers. 

%Amazon echo deployed in 8 older adults’ home over 6 months. Interaction barely goes beyond single commands so not really a conversation \cite{trajkova2020alexa}. 

To address a specific health-related need, a study focused on pain self-management among aging adults using Google Home Assistant. Fifteen community-dwelling older adults with chronic pain participated in a four-week study. The average age of participants was 65 years (55 or older). The voice assistant was used to set reminders for pain management. Participants found the reminders to be consistent, easy to configure, and helpful in promoting accountability for pain management \cite{shade2020voice}.

%Pain self-management in aging adults through reminders using Google home assistant. 4 weeks study. Fifteen community-dwelling older adults with chronic pain and an average age of 65 years (>=55) used the voice assistant for 4 weeks. Reminders were  perceived as consistent, easy to set up, and helpful for accountability \cite{shade2020voice}.

One study used Conditional Voice Recorder (CVR), depicted in that is activated when a proximate Echo is used. When
the ‘wake word’ Alexa is detected, the CVR saves the prior minute and records one further minute of audio (this period is extended if the wake word is heard in the subsequent minute). The CVR also features a button to turn off audio capture, and two LEDs (blue and red), that indicate when the CVR is listening (blue) and when it is recording (red). They did a month long study in 5 households for family oriented smart speaker use.
\end{comment}

%\subsection{Conversational Failures}
\begin{comment}
    

Crowdsourced dataset of failures from Mturk. 199 failures from 107 voice assistant users. Mixed-methods approach.  Conducted interviews. Conducted survey of impact of failures on user trust and their willingness to use in future \cite{baughan2023mixed}
Participants are more forgiving of failures due to spurious triggers or ambiguity of their own request. Failures due to ambiguity occurred when there were multiple reasonable interpretations of a request, and the response was misaligned with what the user intended while still accurately answering the question. Users tended to blame themselves for these failures.
However, failures due to overcapture more severely reduced users’ trust, as when the voice assistant continued listening without any additional input, users considered their use a waste of time compared to errors that users could forsee, understand and work around.
Resumed tasks that they gave up on again after trust was rebuilt by accomplishing much simpler tasks.
Attention failures (activation errors): failures due to spurious triggers are least detrimental. Understanding are most.
Understanding failures maintained highest level of user trust
Response failures: inaccurate action/info lowest perception of integrity. No action is more tolerable.
More to less trusting to: play music -> text a coworker  -> transfer money.

%automatic  evaluation of voice, assistant. this paper talks about measuring user satisfaction as a way to see if errors  have occurred. Their research question is whether you can tell based on user interaction that user was satisfied or not https://dl.acm.org/doi/pdf/10.1145/2736277.2741669. 


%https://www.sciencedirect.com/science/article/pii/S0747563220302181 voice, assistants, and kids mainly about how voice assistance and humans are treated differently in a scavenger hunt. 


\subsection{Background summary}
Data collection done 
\begin{itemize}
    \item using usage logs (no audio files) 
    \item Diary methods
    \item Daily phone call check-ins
    \item Continual (weekly/biweekly) semi-structured interviews (video recorded)
    \item Focus groups

\end{itemize}
Background summary: Tasks and actions [3] are shown in Fig \ref{fig:summary-backfround}

\begin{figure*}[t]
     \includegraphics[width=\textwidth]{summary-background.jpg}    
     \caption{Background Summary: Tasks and actions[3]}
    
    \label{fig:summary-backfround}
\end{figure*}


%Older adults wanted to have conversational style of interaction which despite failures and being aware of limitations of VAs ---lack of follow up and turn by turn interaction due to missing contextual information and conversational history---after significant usage \cite{pradhan2019phantom}. VAs' lack of remembering context after pauses in ``conversations'' with older adults causes frustrations \cite{pradhan2019phantom}.
%Therefore, many interactions remain command-based, suggesting a transactional relationship rather than a conversational one \cite{trajkova2020alexa}. Because of lacking capabilities of VA, researchers in prior work are also reluctant in calling interactions with VAs as a ``conversation'' \cite{porcheron2018voice}. 

%Lack of holistic analysis of on-ground user-VA interactions due to missing real-world audio interaction data make it difficult to interpret concretely to what extent older adults are aware of VA capabilities and what level of effort they put in to recover from conversational breakdowns resulting from their mental model mismatch and other factors such as speech recognition errors due to speech difficulties in older adults \cite{kim2021exploring}. 
%Therefore, further in depth analysis of VA failures with older adults is needed to better understand on-ground complexities. 
%Therefore, in this work, we record audio interactions to capture older adults situated interactions and their immediate reactions and responses to VA actions, specifically informative during erroneous interactions. 

%Voice assistants show significant potential to enhance their quality of life . VAs have been shown to uplift spirits, provide mental engagement opportunities, and aid in fostering social connections for older adults \cite{upadhyay2023studying}.
%slower to adopt \cite{vaportzis2017older, czaja2006factors} but willing to learn and adapt if they see value \cite{heinz2013perceptions}
%Review till 2021: 22 studies included. 18 on Amazon Alexa, 4 novel. Most studied usability and acceptance. Weather, information retrieval and reminders \cite{arnold2022does}. 

%The depth of interaction with these devices varies. For instance, while features such as Alexa's skills can enrich engagements \cite{pradhan2020use}, many interactions remain command-based, suggesting a transactional relationship rather than a conversational one \cite{trajkova2020alexa, purao2019data}.
%On a practical note, voice assistants have showcased significant potential as health aids. In studies focusing on specific needs, such as pain management, older adults found these devices especially beneficial. The voice assistants' ability to set consistent reminders and promote accountability in health routines has been particularly appreciated \cite{shade2020voice}. Customized voice assistant or medical/healthcare data conveyance \cite{shalini2019development}. 
%Moreover,  how they formulate queries to address VAs for healthcare information seeking \cite{brewer2022empirical}. %n=35 scenerio-based interviews and n=201 survey

%Prior work, for example, interviews to identify challenges on quality-of-life enhancements and care delivery. Features used: reminder for medication, event reminders, time inquiry, navigation, playing music, storytelling, news, weather inquiry, appliance control, General Q/A \cite{chen2021understanding}. %[2]. 
%Semi structured interview. By interviewing 16 older adults s (age, M = 76.56, SD = 6.97, 65-90 seems from graph) living independently or semi–independently and 5 providers \cite{chen2021understanding}.
%Prior work, for example, 8 focus groups, with 38 older adults living in a Life Plan Community and who were members and aspiring members of an Amazon Echo program for early adopters \cite{trajkova2020alexa}. Limited value or benefits, beliefs about ability/independence and negotiating use in shared spaces are main reasons for nonuse of echo. However, VAs in future can support independent living, wellbeing and healthy living, and connection with community, resources and people, there are challenges that need to be addressed.  
%Participants ages ranged from 67 to 97 years (M = 81, SD =6.93). Thirty-six participants were members of an early adopters’ program supported by the LPC and, at the time of the interview, had at least one Echo in their homes for at least one year. Two participants had not adopted an Echo but joined the focus groups to hear and share concerns \cite{trajkova2020alexa}. 
%https://journals.healio.com/doi/epdf/10.3928/00989134-20210310-03


%To date, researchers have explore older adults interactions with commercial voice assistants in their homes over extended period of time to understand VAs integration into their lives, VA's benefits, challenges they face and their perception of experience \cite{kim2021exploring, pradhan2019phantom, pradhan2020use, trajkova2020alexa}. 
%Failures and conversational breakdowns during such interactions creates challenges in adoption and continued use of VAs \cite{kim2021exploring, pradhan2020use}.
%However, there is  little  on understanding conversational breakdowns for older adults  \cite{kim2021exploring, pradhan2020use}. The detailed analysis on errors and their resolution is usually missing because of how interactions (specifically erroneous ones) are logged  vaguely in usage logs such as ``text not available'', ``unknown'', ``audio not transcribed'', or  ``Sorry, I don't know about that'' \cite{pradhan2020use}. Thus, usage logs do not effectively capture the continuity of conversation and lack users' in-the-moment reactions and responses.  Moreover, automatic speech detection errors can usually not be picked and categorized just from the transcribed usage logs \cite{kim2021exploring}.  

%Our research is pioneering in its use of long-term, at-home audio data to understand older adults' immediate reactions and responses during VA interactions. Such reactions, including talking over the VA, interrupting, laughing, or murmuring, can provide insights into user satisfaction, frustrations and perceptions of the VA.
%Prior work has shown that additional voice recorder to capture such aspects when looking at how a family interacts with smart speakers in beneficial in understanding their interaction and experiences \cite{porcheron2018voice}.
%And Similar to how users' facial reactions can help identify conversational breakdowns \cite{cuadra2021look}, we explore if we can gather users' verbal and vocal responses to erroneous interactions as that is more practical and feasible for purely voice based interactions. 

%Using the real-world audio interaction data, we can accurately capture and classify these errors, and see instantaneous responses or actions taken by users to identify and fix the errors, whether they recover from errors at all and if so in how may retries. Altogether to give a holistic and nuanced view of erroneous interactions and older adults challenges around errors in the real-world long-term interactions.
%While,  the commercial voice assistants such as Alexa now has follow up mode for continued conversation but the audio is mostly categorized as not intended for Alexa, or  not properly utilized (vocal and verbal cues) to improve user experience specifically when breakdowns occur. 


%To the best of our knowledge no prior work directly uses audio data for interactions for long-term at home interactions for older adults to understand immediate reactions and responses of users while VA is responding i.e., talking over the VA, interrupting the VA, laughing or murmuring, and other vocal and verbal response. Such reactions during and immediately after the interaction with VA can be beneficial in understanding their satisfaction to VA's response, and perceptions of VA. 
%Thus, in this work, we qualitatively look at \emph{how users' react to VAs immediately using vocal or verbal cues  and how can we improve human-agent interaction by using users' immediate reactions or responses specifically around conversational breakdowns?}


%Limitations of voice assistants in understanding context and keeping track of conversation. Traditional Natural Language Processing (NLP) such as keyword-based recognition can be more hindering for older adults since they prefer more natural human communication  \cite{pradhan2020use, pradhan2018accessibility}. Moreover, most interactions remain one turn and do not go beyond that \cite{purao2019data} Moreover, there may be more automatic speech recognition errors for older adults because of speech difficulties such as slower speech, stuttering, pauses, repeats, stretching, incomplete or false syntactic structures \cite{kim2021exploring} thus making traditional NLP tools further ineffective. 
%Large Language Models (LLMs) are being integrated in VAs and explored to understand how they improve user experience for various applications such as healthcare \cite{jo2023understanding, yang2023talk2care, mahmood2023llm}, conversational recommendar systems \cite{qu2023towards, mahmood2023llm} and other assistive tasks such as cooking \cite{chan2023mango}. LLMs have shown to be  useful at interpreting more natural, faulty, vague and conversational intents \cite{mahmood2023llm} which can be particular beneficial to improve older adults experience with VAs. Therefore, we build and deploy an LLM powered voice assistant i.e., integrating ChatGPT into Alexa skills as a technology probe \cite{hutchinson2003technology} after 2 weeks in our 4 week study to understand the potential benefits and challenges of an LLM-powered VA on the ground with older adults. The integration of LLMs and voice interfaces in publically available platforms such as  ChatGPT \cite{OpenAI2023} and specifically Amazon Alexa \cite{alexaLLM2023} for various applications makes this exploration timely to understand how these futuristic technologies can be tailored for special population such as older adults. 



%CM: Technology probe could be a good way to frame your deployment project:
%Amama: for chatGPT integration into the Alexa part... https://dl.acm.org/doi/abs/10.1145/642611.642616 and https://dl.acm.org/doi/abs/10.1145/2556288.2557416

%nuanced interactions around errors. Therefore, we also look at  \emph{what types of conversational failures and errors occur when older adults interact with VAs, how do they react or respond to those errors? how they recover from such errors, are there multiple retries to recover from error? how many errors are resolved and after how many tried} altogether 

%do not make use of vocal and verbal cues fully to improve the interaction,
%Voice interactions are improved by taking other verbal and vocal cues into account. For instance, verbal back-channels in turn-taking conversations are informative of understanding, acknowledgement, exemplification and much more. 

%timely since Alexa is now capturing instant user response in some sense but mostly categorizes it as not intended for Alexa or just doesn't use it effectively to improve so far at least in their follow up mode
%Researchers study potential use of such cues in lab settings (citations).. However, 
%\section{Research Context}

%However field studies with older adults, usually done using commercial smart speakers, do not have audio recorded data of the whole interaction to capture social cues and reactions fully.
%Prior research for understanding older adults' interaction with VAs mainly relied on usage logs,diary methods, daily phone call check-ins, continual (weekly or biweekly) semi-structured interviews (recorded videos), and focus groups. Usage logs do not effectively capture the continuity of conversation and lack users' in-the-moment reactions and responses. 

\begin{comment}
    


\subsection{Research Questions}
\begin{itemize}
    \item What are the services that are most used and what services that they stopped using over time and try to understand the reason for continued/discontinued use of specific features of VA? Try to categorize the conversations into categories such as functional, entertainment, social e.t.c.
    \item  What types of conversational failure occur and who the user blames for such errors? Can we classify user reactions and map those to types of failures? Severity of failures and responses based on that? Taxonomy of failures and users' responses.
    \item How can we use users' immediate vocal or verbal reactions to capture conversational breakdowns, improve recovery from such breakdowns (proactive recovery?), and continue conversations intelligently by taking users' feelings (happy, frustration, angry e.t.c.) into account. In short, how can we improve UX by using users' immediate reactions or responses?
\end{itemize}

\end{comment}

%\subsection{Contributions}


%While 4-week study provided ample insights into older adults situated social behavior towards VAs, specifically during breakdowns, longer interactions over months can be more informative. also can be used as a way to gather data to train VAs to be better at error identification and recovery. 

%We only look at query and responses for now qualitatively to identify potential of its use, detailed query analysis such as in \cite{brewer2022empirical} can be beneficial to further understand older adults interactions. 

%We explored generic use case of LLM-powered VA in this study, however, specific application such as healthcare information seeking or support for older adults with disabilities and impairments can be explored more in future. Moreover, our participant sample is small and limited, greater sample size with varied abilities needs to be explored. 

%Traditional voice assistants have missed the opportunity to effectively utilize instantaneous user reactions, explicit actions to fix errors, and conversation history in VAs' recovery from errors or in assiting users to recover from errors. In this qualitative longitudinal study, we captured such immediate user responses and reactions through an audio recorder and demonstrated  that most errors can be identified from users' responses and actions to errors. Moreover, we showed that need for scripted commands and well-formed queries increases the conversational breakdowns for older adults due to their inaccurate mental model of VA capabilities, forgetfulness of query styles that work and want to use more naturalistic style of communication. We further explored the potential of LLM integration into Alexa to enhance the conversational capabilities of VAs for older adults. Our findings offer insights and consideration for design and research of nuanced interaction dynamics of older adults with futuristic conversational voice assistants through ``in-the-wild'' data collection. 

VA related 3 questions

health 7 questions

history 6 
planning trip (specific places) 2
what's the good music to help me relax
is the extreme heat ummm natural to weather" 

story 2

food and drink 1

may be we can have a questionnaire/ part of interview dedicated to understanding types of errors they faced and who they assigned the blame to, themselves or the speaker. We will have access to their usage log before we go in for the exit interview. May be we can gather and categorize the failures and talk about those in semi structured interview


\begin{figure*}[t]
     \includegraphics[width=\textwidth]{figures/error distribution.png}    
     \caption{Error rates for each interaction type (erroneous interaction/total interactions for each type). Left is a pie chart of the type of interaction vs. error. The right graph shows that within information seeking, types of questions that contribute to errors. The number within pie chart shows number of errors in that category and percentage it contributes to total erroneous interactions of question type. For instance, local information had 31 errors which is $17.6\%$ of all errors ($n=31$ of 176) in question type. The arrows show the percentage of type of question queries that ran into error (error rate for each type of questions). For instance, $59.62\%$ of total local information questions resulted in error ($n=31$ out of 52).}
    
    \label{fig:errors-distribution}
\end{figure*}


%were of wide variety such as negation, laughter, acknowledgment, negative comments and even positive comments and gratitude (see Table \ref{tab:errors-reactions}). Such span of reactions of social nature indicate more than just a transactional interaction with the VA. 

%The immediate responses and audio interactions captured through our recording device provide insights into the extent of this integration, offering a nuanced perspective on their daily use of VAs.


\subsection{Design Considerations for LLM-powered VAs for Older Adults}
In exploring the interactions of older adults with LLM-powered VAs, our findings provide insights into such VAs' conversational capabilities and resilience to errors. Based on these insights we highlight opportunities, challenges, and provide design considerations for future LLM-powered conversational VAs for older adults. 

\subsubsection{Enhanced VA conversational capabilities and older adults learning curve}

The integration of LLMs into VAs significantly enhances their conversational abilities for information retrieval. Such LLM-powered VA maintains context and conversational history, enabling users, to ask follow-up questions and engage in multi-turn interactions with reduced friction \cite{mahmood2023llm}. 
For example, P15 demonstrated such enhanced interaction by asking a follow-up question, ``Why should I keep the room dark,'' after receiving the said advice on falling asleep (refer to C16 in Table \ref{tab:alexa-dialogue-chatGPT}). This ability to maintain context and respond to vague, more conversational queries represents a substantial improvement in VA-user interaction for older adults.

Additionally, our observations indicate that older adults, such as P15, become more adept at interacting with the ChatGPT-powered Alexa with practice. Comparing P15's initial interaction in the afternoon (C15 in Table \ref{tab:alexa-dialogue-chatGPT}) with a later one in the evening of the same day (C17 in Table \ref{tab:alexa-dialogue-chatGPT}) reveals a more fluid conversation, suggesting a learning curve. Improvement after trial and error in user interaction with such advanced VAs highlights the critical role of guidance for older adults in their initial usage stages. To facilitate this familiarization process and improve their overall experience, it is beneficial for VAs to provide instructive tutorials and helpful tips during interactions. For example, incorporating suggestions like, ``By the way, you can ask me follow-up questions without having to say the keyword,'' or informative prompts such as, ``I can answer any questions regarding history, technology, and can fetch recipes,'' can significantly aid users in understanding the breadth and depth of the VA's capabilities. Such approach not only makes the technology more accessible but also empowers users to make the most of their VA interactions.

\begin{adjustwidth}{0.3cm}{0pt}

    
    \textbf{Opportunity 2:}
    \textit{LLM-powered VAs can enhance older adults experience for information retrieval.}

    \noindent
    \textbf{Opportunity 3:}
    \textit{Learning curve in older adults using advanced VAs reveals an opportunity to enhance user experience through trial and error.}
    
    \noindent
    \hl{\textbf{Design Consideration 7:}
    \textit{Embed instructive tutorials and tips in VA interactions to help older adults effectively use advanced voice assistant features.}}  


\end{adjustwidth}   


 

\subsubsection{Conversational resilience}
\label{sec:discussion-LLM-conversational resilience}
%Seamless integration is essential for older adults using VAs, as our study shows that additional steps for skill activation can act as barriers for adoption and use of ChatGPT-powered Alexa skill. Most errors in these interactions were noted at the skill activation level, particularly during attempts to exit the skill (section \ref{sec:chatGPT-interactions}). To improve user experience, VAs should not require explicit activation and should use natural language for skill closure and termination to enable more intuitive and user-friendly interactions, specifically since older adults tend to be forgetful as discussed in section\ref{sec:discussion-forgetfulness}.


%In interactions involving ChatGPT, we observed that all intent recognition errors were regarding the misinterpreting users' intent to exit the Alexa skill rather than ChatGPT's understanding of user intent, indicating ChatGPT's high level of accuracy in understanding user requests. 
In interactions with ChatGPT, all intent recognition errors related to misinterpreting participant intent to exit the Alexa skill, not ChatGPT's understanding of their intent, highlighting its high accuracy in comprehending user requests.
Most errors were related to Alexa's speech technology and skill activation level, particularly during attempts to exit the skill, yet the overall intent was accurately identified in most cases (see section \ref{sec:chatGPT-interactions}). Notably,  errors in ChatGPT skill interactions were often resolved within a maximum of two retry attempts by participants, showcasing better error resolution compared to standard Alexa interactions where many errors remained unresolved despite multiple retries as shown in section \ref{sec:errors-retry}.

However, we identified issue of partial listening errors, particularly prevalent among older adults as they may take longer to formulate their queries (C13 Table \ref{tab:alexa-dialogue-chatGPT})---suggesting a need for improvement in Alexa's voice interface to better accommodate users with slower speech patterns and speech difficulties.%, as illustrated in conversation 
Given that interactions with LLM-integrated VAs tend to be more conversational and the responses more verbose \cite{mahmood2023llm}, it is crucial for these systems to allow ample time for users, especially older adults, to process the information and articulate their queries. Adaptions to user speech rate and context would ensure that voice user interfaces (VUIs) are more aligned with the communication styles and needs of older users, enhancing the overall usability and effectiveness of the technology.





\begin{adjustwidth}{0.3cm}{0pt}

    
    \textbf{Opportunity 4:}
    \textit{Enhanced error resolution and intent recognition in VAs with LLM integration can be beneficial for older users.}

    \noindent
    \textbf{Limitation 6:}
    \textit{Limited adaptability of VUIs for current assistants to slower speech patterns and extended speaking time needs of older adults especially when VAs are more conversational.}
    
    \noindent
    \hl{\textbf{Design Consideration 8:}
    \textit{Tailor VUIs to better suit the conversational pace and preferences of older adults, ensuring more fluid conversational interaction.}}  


\end{adjustwidth}   



%Despite being aware of VAs' limitations to an extent---the lack of follow-up and context in interactions---older adults still desire a conversational style and originally follow that \cite{pradhan2019phantom}. However, VAs' inability to retain context also leads to frustration\cite{pradhan2019phantom}. Thus, older adults' expectations for conversational and human-like interactions with VAs lead to breakdowns during information retrieval (health-related) causing them to resort to rephrasing their queries to more scripted and self-contained against their preference \cite{brewer2022empirical}.
%Consequently, many interactions with VAs are still predominantly command-based, suggesting a transactional rather than conversational relationship \cite{purao2021use}. This transactional dynamics leads researchers to question whether these interactions can truly be classified as ``conversations'' at all \cite{porcheron2018voice}.

\section{Introduction}
Voice Assistants (VAs), despite their growing popularity, often are not designed for special populations such as older adults \cite{stigall2019older}. However, older adults tend to prefer speech over text-based modalities when interacting with technologies \cite{kowalski2019older, wulf2014hands, liu2020design, choi2020use}, suggesting that VAs could enhance their quality of life and autonomy \cite{smith2023smart, blair2019understanding}. 
Researchers have investigated older adults' long-term interactions with VAs at home, focusing on their adoption, benefits, challenges, and perceptions \cite{kim2021exploring, pradhan2019phantom, pradhan2020use, purao2021use}.  
Nevertheless, the adoption and sustained use of VAs are impeded by AI failures and errors \cite{kim2021exploring, pradhan2020use}, which are particularly more prevalent for older adults partly because of their verbose and disfluent speech patterns \cite{mortensen2006age}.
%since they tend to be verbose and show more disfluency in speech compared to young adults 
A significant research gap exists in comprehensively analyzing these errors and their resolution, largely due to insufficient error logging in usage data (``text not available'' or ``unknown'') \cite{pradhan2020use} which lacks conversational context and real-time user reactions. Furthermore, speech recognition errors are often not identifiable solely from transcribed usage logs \cite{kim2021exploring}. Even though commercial VAs (Alexa, Siri) have a follow-up mode for continuous conversation, the audio is frequently misclassified (``Audio not intended for Alexa'') rendering it underutilized, especially during conversational breakdowns.
%thus, not effectively utilized, especially during conversational breakdowns.

In contrast, supplementary audio recordings have proven effective in capturing nuanced aspects of interactions with smart speakers in family settings \cite{porcheron2018voice}. 
Consequently, we explore whether \textit{``in-the-wild'' audio interaction data can provide richer, more contextually grounded insights into older adults' behavior and interaction dynamics, particularly focusing on error identification, conversation progression, and the overall efficacy of VAs in their lives}.
To achieve this, we deployed Alexa smart speakers along with developed audio recorders in the homes of older adults for four weeks, allowing us to capture and analyze users' verbal and vocal responses during and immediately after interactions with Alexa. The evaluation of the real-world audio data not only shed light on their overall interaction dynamics but also enabled a detailed analysis of conversational breakdowns. 
%Our findings not only shed light on the overall interaction dynamics\cmh{seems repetitive; similar to the previous sentence} but also highlight the potential of users' immediate reactions and corrective actions in facilitating error recovery processes, ultimately enhancing the user experience.

\cmh{do not flow well with the previous paragraphs. What if we begin with clearly stating two research questions that we want to answer in this work and structure the intro this way. Can talk more on Thursday coffee chat.}
One major limitation of current VAs is their inability to understand context and maintain conversational flow,  resulting in most interactions being restricted to a single turn \cite{purao2019data, purao2021use}. Traditional Natural Language Processing (NLP) methods, such as keyword-based recognition that require somewhat scripted user queries, are less effective for older adults who prefer more natural communication \cite{pradhan2020use, pradhan2018accessibility}. This limitation is exacerbated by the prevalence of speech recognition errors in this demographics due to factors such as slower speech stuttering, pauses, repeats, stretching, incomplete or false syntactic structures \cite{kim2021exploring}. 

On the contrary, Large Language Models (LLMs) have shown promise in interpreting natural, faulty, and conversational intents \cite{mahmood2023llm}, which could significantly improve older adults' experiences with VAs. \textit{To explore the potential benefits and challenges of an LLM-powered VA in-the-wild with older adults}, we integrated ChatGPT into Alexa skills as a technology probe  \cite{hutchinson2003technology} after two weeks of our four-week study.after two weeks in our four week study. 
The integration of LLMs and voice interfaces in publicly available platforms such as Alexa \cite{alexaLLM2023} makes this exploration pertinent to understanding how these futuristic VAs can be tailored for special populations like older adults. 
%The announcement of integration of LLMs and voice interfaces in %publicly available platforms such as  ChatGPT \cite{OpenAI2023} and  Alexa
%\footnote{Implementation and data collection for this study was conducted before this announcement.} \cite{alexaLLM2023}  makes this exploration timely to understand how these readily available futuristic VAs can be tailored for special population such as older adults. 
Our findings emphasize the resilience of LLMs in conversation and the learning curve for older adults to achieve improved interactions, providing key design insights for future LLM-powered VAs. 
Contribution of our work is three-folds:

\begin{enumerate}[leftmargin=*]
    \item \textbf{Thematic analysis of real-world interaction data:} Detailed thematic analysis of the real world audio interaction data to understand how VAs fit into the lives of older adults, the nuances of the  erroneous interactions, and the challenges they face. We highlight opportunities and limitations to offer design considerations for enhancing VA interactions for older adults. 
    \item \textbf{LLM-powered VA as a technology probe:} Developed, deployed and evaluated an LLM-powered VA as a technology probe to understand how older adults interact with highly conversational, futuristic VAs to identify opportunities and limitations of LLM integration into VA technology. 
    \item \textbf{Methodology---data collection tool:} Introduction of a novel method to collect ``in-the-wild'' audio data, enabling a deeper understanding of user interactions with, and perceptions of VA within their personal environments. 
    
\end{enumerate}

Commercial Voice 

Assistants (VAs), despite their growing popularity, are not designed for special populations such as older adults \cite{stigall2019older}. However, older adults tend to prefer speech over text-based modalities when interacting with technologies \cite{kowalski2019older, wulf2014hands, liu2020design, choi2020use}, suggesting that VAs could enhance their quality of life and autonomy\cmh{the connection between preferring speech modality and the potential of va in improving quality of life is unclear} \cite{smith2023smart, blair2019understanding}. 
Researchers have investigated older adults' long-term interactions with VAs at home, focusing on their adoption, benefits, challenges, and perceptions \cite{kim2021exploring, pradhan2019phantom, pradhan2020use, purao2021use}\cmh{revisit: need a better way to connect with the previous sentences and the next one}.  
In this study, we aim to expand upon the existing understanding of how older adults interact with voice assistants in their homes by exploring two key questions:

%\noindent \textbf{RQ1: How ``in-the-wild'' audio interaction data can provide richer, more contextually grounded insights into older adults' behavior and interaction dynamics, particularly focusing on error identification and conversation progression?}
\textbf{RQ1: How can audio interaction data captured in the wild offer deeper, context-rich insights into the behaviors and interaction dynamics of older adults with VAs, particularly in identifying errors and advancing conversations?}
The adoption and sustained use of VAs by older adults are impeded by AI failures and errors \cite{kim2021exploring, pradhan2020use}, which are particularly more prevalent for older adults partly because of their verbose and disfluent speech patterns \cite{mortensen2006age}.
A significant research gap exists in comprehensively analyzing these errors and their resolution, largely due to insufficient error logging in usage data (``text not available'' or ``unknown'') \cite{pradhan2020use}. This shortfall often leaves conversational context and real-time user reactions unrecorded. Furthermore, speech recognition errors are often not identifiable solely from transcribed usage logs \cite{kim2021exploring}. Although commercial VAs (Alexa, Siri etc.) offer a follow-up mode for ongoing conversation, the audio is frequently misclassified (``Audio not intended for Alexa'') rendering it underutilized, especially during conversational breakdowns. 
In contrast, supplementary audio recordings have proven effective in capturing nuanced aspects of interactions with smart speakers in family settings \cite{porcheron2018voice}. %MAKE IT MORE EXPLICIT like because they cannot study it
Therefore, to investigate the additional insights offered by ``in-the-wild'' supplementary audio data of older adults' interactions with a VA (RQ1), we deployed Alexa smart speakers along with developed audio recorders in their homes for four weeks. This audio data allowed us to capture and analyze users' verbal and vocal responses during and immediately after interactions with Alexa, shedding light on their interaction dynamics and providing a comprehensive analysis of conversational breakdowns.

%The evaluation of the real-world audio data not only shed light on their overall interaction dynamics but also enabled a detailed analysis of conversational breakdowns. 


\textbf{RQ2: What potential benefits and challenges does an LLM-powered VA present in enhancing the interaction quality for older adults, addressing the limitations of current commercial voice assistants?}
%We see that these A key limitation of current VAs is their struggle with understanding context and maintaining a flow in conversation, often restricting interactions to a single exchange \cite{purao2019data, purao2021use}. Conventional Natural Language Processing (NLP) methods, which rely on somewhat scripted user inputs, fall short for older adults who prefer more natural forms of communication \cite{pradhan2020use, pradhan2018accessibility}. This limitation is exacerbated by the prevalence of speech recognition errors in this demographics due to factors such as slower speech stuttering, pauses, repeats, stretching, incomplete or false syntactic structures \cite{kim2021exploring}. 
Nevertheless, large language models (LLMs) have demonstrated potential in interpreting natural, flawed, and conversational speech \cite{mahmood2023llm}, which could significantly improve older adults' experiences with VAs. Therefore, to explore the potential benefits and challenges of an LLM-powered VA in-the-wild with older adults (RQ2), we integrated ChatGPT into Alexa skills and deployed as a technology probe  \cite{hutchinson2003technology} in the latter half of our four-week study.
The integration of LLMs and voice interfaces in publicly available platforms such as Alexa \cite{alexaLLM2023} underscores the relevance of this exploration in understanding how advanced VAs can be tailored for special populations such as older adults. 
Our findings emphasize the resilience of LLMs in conversation and the learning curve necessary for older adults to engage effectively with such sophisticated VAs, providing crucial insights for the design of future LLM-powered VAs. 


Contribution of our work is three-folds:

\begin{enumerate}[leftmargin=*]
    \item \textbf{Empirical---Thematic analysis of real-world interaction data:} We conduct an in-depth thematic analysis of ``in-the-wild'' audio interaction data to understand how older adults incorporate VAs into their lives, especially focusing on the nuances of erroneous interactions. Our findings reveal both opportunities and challenges, offering valuable design guidelines for creating more robust and fluid VA interactions.
    \item \textbf{Methodology---Data collection tool:} We introduce a novel method for collecting ``in-the-wild'' audio data, enabling a deeper understanding of how users interact with and perceive VAs within their personal environments. %user interactions with, and perceptions of VA within their personal environments. 
    \item \textbf{Empirical---LLM-powered VA as a technology probe:} We develop, deploy, and evaluate an LLM-powered VA as a technology probe to understand how older adults engage with conversationally adept futuristic VAs to identify opportunities and limitations of LLM integration into VA technology for older adults. 
    
\end{enumerate}




\section{Abstract}
Commercial Voice Assistants (VAs), though promising to benefit older adults, face adoption challenges due to errors and lack of contextual understanding. Traditional methods of capturing user experience---usage logs and post-hoc interviews of user perceptions---lack depth in capturing nuances of user-VA interactions, particularly regarding errors and breakdowns.
To address this limited understanding in the literature, we deployed Amazon Echo smart speakers with custom audio recorders in the homes of $15$ older adults for a four-week study, capturing ``in-the-wild'' audio data, including overlapping speech and immediate user responses.
We observe the social integration of VAs in users' lives, as demonstrated by participants interactions with each other and participants showing Alexa off to their guests.
Moreover, our qualitative analysis reveals the potential of employing user state, evident in their immediate responses, to improve VA error handling. Additionally, older adults exhibited an inaccurate mental model of VA capabilities, preferring a more naturalistic query approach which current VAs cannot fulfill. 
To address such conversational limitations of VAs, we explore integration of Large Language Models (LLMs) into Alexa as LLMs have shown promise in recognizing natural, conversational, and even faulty speech patterns. After two weeks of the 4-week study, we deployed a ChatGPT-powered Alexa skill to assess its effectiveness for older adults in information retrieval. Our findings underscore the resilience of LLMs in maintaining conversational flow and highlight the learning curve for older adults in adapting to more advanced VAs. Finally, we suggest considerations for designing VAs better attuned to older adults' needs, enhancing their interactions and integration into daily life.
\subsection{Aligning Older Adults' Expectations and Voice Assistant Functional and Comprehension Abilities}
%\subsection{Adjusting Older Adults' Expectations and Advancing VA Functionality and Comprehension}
%\subsection{Shaping Older Adults' Expectations and Enhancing Voice Assistant Functional and Comprehension Abilities}


Our findings indicate that participants often overestimate or underestimate VA capabilities. However, VAs struggle to capture the natural speech patterns of older adults highlighting a need to enhance VAs' ability to understand user intentions. The continuous advancement in VAs' functional and comprehension capabilities, necessitates an active recalibration of older adults' mental models for optimal technology use. In the following discussion, we explore and present design considerations evident from our findings for both adjusting the mental models of older adults and improving VA comprehension of their intent.

%Our results have shown that participants over or underestimate VA capabilities and VA is unable to capture older adults natural way of speaking while older adults. There is need for increasing VA capabilities to understand user intentions. The evolving improvement in both VAs functional and comprehension capabilities (for instance potential of LLMs) calls for active calibration of  older adults mental model to optimize their use of technology. Below, we discuss how to achieve both fixing mental model of older adults and improve VA's comprehnsion. 

\subsubsection{Inaccurate mental model of VA capabilities}
\label{sec:discussion:mental-model}
Our study reveals a notable discrepancy in participants' understanding of voice assistant capabilities, leading to an inaccurate mental model. The high incidence of limitation errors ($n=130, 20.6\%$), where the VA fails to fulfill user intents and responds with ``I don't know about that'' (see Table \ref{tab:errors-def}) , illustrates that Alexa often cannot meet older adults' requests. Occurrence of limitation errors, thus, suggest that older adults may not be fully aware of the VA's capabilities, especially regarding how to formulate their queries that Alexa can comprehend. %particularly in terms of what Alexa can understand in terms of formulating queries. 
Additionally, certain interaction types with VAs exhibit notably higher error rates, particularly in less frequent, 'edge' categories such as miscellaneous queries, TV-related commands, stories, and poems (see Figure \ref{fig:errorneous-interactions}). Such trend extends to less commonly asked questions pertaining to famous people,
%\cmh{famous personalities?}, 
Alexa itself, history and specific places that had error rates exceeding 50\% (refer to Table \ref{tab:question-type}). Similarly, Miscellaneous queries that did not fit other categories also had high error rate of 44.47\%. 
The high error rates in less common interactions and questions further emphasize the mismatch between user expectations and VA capabilities underscoring the necessity for VAs to either adapt more effectively to a broader range of user queries and commands, or to communicate their capabilities in a clearer manner.
%Evidence of high error rates in less common interactions and questions further highlights disparity between user expectations and VA capabilities, underscoring the need for VAs to adapt more effectively to a wider variety of user queries and commands or at least be able to communicate the uncertainity in a better way

The disconnect between user mental models and VA capabilities becomes more apparent upon examining example interactions between couples with divergent mental models. For instance, in the case of P11, the couple demonstrated differing perceptions: P11a overestimated the capabilities of Alexa (C8 Table \ref{tab:alexa-dialogue-private-conversations} and C11 Table \ref{tab:alexa-dialogue-errors}), whereas P11b underestimated them (C6). Such disparities in understanding were not isolated; several participants either overestimated or underestimated the VA's functionalities.
Instances of overestimating were also observed with individual participants such as P8 attempting to access TV channels through the VA and P2 asking the device to remember their conversations (C10 in Table \ref{tab:alexa-dialogue-errors}). Moreover, P6 requested an example of a meme, highlighting a misconception about the VA's ability to convey visual information verbally (C19 Table \ref{tab:alexa-dialogue-additional}). Questions about Alexa's capabilities, such as P11b asking if it could speak in a British accent or P2 questioning the extent of its conversational memory (C10), further illustrate how participants are unaware of its capabilities and tend to directly ask the VA.
 
%prior work showing that users rely on trial and error to form mental model of how VAs work \cite{kim2021exploring}. 

Regular users of multiple smart speakers for many years still had misconceptions about VA's capabilities. For instance, P1 attempted to control non-smart, unconnected lights via Alexa reflects a fundamental misunderstanding of the technology's requirements and limitations. Additionally, the same participant's habit of commanding Alexa to stop talking even after it had finished indicates a cautious approach (underestimating VA capabilities), stemming from uncertainty about controlling the device. Such behavior was also noted in the participants who are new users, suggesting a broader trend of over-caution (saying ``stop'' when not necessary or saying ``stop'' multiple times) due to unclear understanding of the VA's operation. 
Our new finding of mental model mismatch in `experienced' users (P1),  highlights that even long-time older adult users may not be fully aware of a VA's capabilities\cmh{repeating the beginning of line 1661?}, including simple commands such as `stop'. Previous research indicates that users often rely on trial and error to develop their mental model of the VA \cite{kim2021exploring}. However, our findings suggest that this method might not always correct their mental model; instead, it tends to reinforce behaviors that `work' rather than those that are more effective and accurate. Consequently, providing both novice and experienced users, particularly older adults who may have a limited grasp of the technology, with accurate information is crucial. 
%Additionally, with recent advancements in the field \cite{OpenAI2023, alexaLLM2023} the capabilities of VAs change swiftly for older adults to have a rigid mental model. There is a need for adaptive methods to actively keep updating their mental model. 
Furthermore, with rapid advancements in the field with the integration of LLMs in voice assistance technology \cite{OpenAI2023, alexaLLM2023}, the capabilities of VAs are evolving too quickly for older adults to maintain a fixed mental model---which calls for dynamic approaches to continually update their understanding of these technologies.

To promote continued use of VAs, it is essential to develop user-focused instructional protocols that offer clear initial guidance and continued learning support across various formats such as online tutorials and in-device instructions \cite{koon2020perceptions}. Dedicated tutorials with real-time updates or corrective actions by VA embedded in daily interactions can be employed to effectively convey the VA's capabilities and optimize older adults use of this technology. 
To address the gap between users' perceptions and the actual capabilities of VAs, it is crucial for VAs to provide more informative responses to users' direct or indirect queries about their functionalities. Enhancing VAs to actively engage older adults in questioning and understanding the VA's functionalities through up-to-date tutorials---both during the adoption phase and consistently over time---can help correct their misconceptions\cmh{how is this different from a previous point/consideration about tutorial?}. 
Moreover, VAs should be designed to detect instances of user misconceptions, responding with tailored information that helps rectify these misunderstandings. Instead of defaulting to generic and uninformative responses such as ``Sorry, I don't know that,'' the VA should provide context-specific explanations \cite{pradhan2020use, kim2021exploring}. For instance, if a user attempts to interact with a non-smart device, the VA should explain the prerequisites for smart home integration, rather than merely stating, ``Sorry, I couldn't find a connected light.'' Such approach not only clarifies the VA's limitations but also educates the user about the necessary conditions for optimal use. Responses should be tailored to accommodate varying levels of technological familiarity, specifically for older adults. 
Such user-aware enhancements in VA interactions will aid in aligning older adults' expectations with the realistic capabilities of the technology, fostering a more accurate and comprehensive understanding of how VAs can be utilized effectively and consistently.



\begin{adjustwidth}{0.3cm}{0pt}

    
    \textbf{Limitation 4:}
    \textit{Lack of conveyance of its capabilities by the VA continually results in inaccurate mental model for older adults even in long-time users.}

    \noindent
    \hl{\textbf{Design Consideration 7:}
    \textit{VAs should employ user-aware and error-aware informative responses in daily interactions along with tutorials at adoption stage to handle mental model mismatch.}}  

    \noindent
     \textbf{Limitation 5:}
    \textit{Rapid advancements in VA technology further exacerbates the gap between the new capabilities and the relatively static mental models of older adults.}
    %Rapid advancements in VA technology quickly outpace the static mental models of older adults.

    \noindent
    \hl{\textbf{Design Consideration 8:}
    \textit{Create dynamic and adaptable tutorials and provide real-time announcements during daily interactions to align older adults' mental models with the evolving nature of VA technology.}}  
   

\end{adjustwidth}   



\subsubsection{Lack of VA's comprehension of users' natural way of speaking}

Our findings highlight a significant gap in Alexa's ability to comprehend the natural speech patterns of older adults\cmh{didn't we discuss this before?}. The high rate of intent recognition errors, where the VA incorrectly responds to user queries ($32.3\%$, $n=204/632$, as detailed in section \ref{sec:error-types-resolution}), reflects Alexa's limited comprehension of user intent that may be attributed to older adults using natural speech patterns rather than crafting scripted, well-formed queries.  For instance, participants often preferred to use more conversational phrases such ``Thank you'' \cmh{didn't we discuss this before?}instead of command-like terms such as ``stop,'' likely perceiving the latter as interruptive or rude. Whereas, some older adults tend to favor polite interactions, both in their own communication with VAs \cite{pradhan2019phantom} and in receiving responses from VAs \cite{hu2022polite}. 
Older adults, such as P15, consistently reverted to natural phrases (``Thank you, I have taken my medicine'') instead of specific commands (``cancel alert'') as illustrated in C12 Table \ref{tab:alexa-dialogue-errors} underscoring a desire for more intuitive interaction with VAs, %(section \ref{sec:}), 
which is especially challenging for older adults as they expect VAs to to possess greater conversational and social capabilities compared to the expectations of younger adults \cite{oh2020differences}. Additionally, the requirement to carefully consider and rephrase queries due to the limited ability of VAs to comprehend diverse speaking styles—acknowledging that not everyone speaks the same language—becomes more pronounced for individuals from varied demographic backgrounds  \cite{harrington2022s}. 
Preference for naturalistic communication over rigid, scripted commands or structured queries is also illustrated by P2, who often had to reformulate queries multiple times in an attempt to elicit the desired response due to Alexa's limitations in understand his intent  as shown in C1 Table \ref{tab:alexa-dialogue-questions} and C10 Table \ref{tab:alexa-dialogue-errors}. Furthermore, compound errors (refer to section \ref{sec:errors-retry}) can further escalate the friction between the user and the VA as illustrated in C1 Table \ref{tab:alexa-dialogue-questions} where P2 keeps reformulating his queries to get the information he wants. 
The failure of voice assistants to recognize user intents not only causes friction between them but can also lead to decreased usage over time, as indicated by our findings (see Fig. \ref{fig:uagaes-over-days}). For instance, P1b discontinued attempts to communicate with Alexa after repeated misunderstandings as illustrated in C20 Table \ref{tab:alexa-dialogue-additional}. 

Such intent recognition failures becomes particularly critical in high-stakes scenarios\cmh{didn't we discuss this before?}, such as medication reminders. P15, for example, relied on Alexa for medication reminders but struggled with informing the device when the task was completed (C12 Table \ref{tab:alexa-dialogue-errors}), often leading to confusion and frustration captured during one of her interactions during the study: ``\textit{I don't know what I am supposed to say to it to tell it that I have taken it}''. Need to use specific keywords is found to be annoying by older adults \cite{pradhan2020use, pradhan2018accessibility}. Despite Alexa having the functionality to track completed reminders, it often failed to understand P15's queries such as ``\textit{Did I take my medicine today?}'' Requiring users to pose rigid commands and well-formulated queries ties back to the previously discussed mismatch in mental models (section \ref{sec:discussion:mental-model}) and is exacerbated by the observed forgetfulness in older adults (section \ref{sec:discussion-forgetfulness}). Older adults reverting to use of their natural style of speech highlights their expectation and preference for VA to be able to comprehend that. Therefore, adapting voice assistants to understand and respond to more naturalistic speech patterns---especially considering the speech difficulties, forgetfulness of older adults, and them being slow in adopting to new technologies \cite{vaportzis2017older, czaja2006factors}---is crucial for enhancing their user experience and ensuring effective communication. 

Intent recognition should be \textit{human-aware}, especially considering the varying speech styles of older adults\cmh{didn't we discuss this before?}, which differ both from other user groups and within the older adult demographic itself. For instance, leveraging people's social cues, verbal and vocal in this case, to infer their implicit intent and creating personas to form a mental model of users can improve the VA's ability to accurately recognize intent.  Being agnostic to users' state---body language, audio-prosodic features and other contextual information---results in voice assistants failing to appropriately respond or react to older adults \cite{cuadra2022inclusion}. Moreover, as evidenced in our exploration of LLM-powered VAs (see section \ref{sec:results-chatGPT-breakdowns}) and as discussed in sections \ref{sec:discussion-levraging-llm} and \ref{sec:discussion-speech-challenges}, utilizing LLMs contextual capabilities (retaining task information, conversation history, and user personas etc.) can further improve intent recognition, particularly in adapting to flexible user query formulation. Such integration of LLMs demonstrates a more effective approach in deciphering user intent \cite{mahmood2023llm}. 
%Better intent recognition from flexible speech styles can also be achieved by employing LLMs to determine user intent as depicted by the results of our exploration of LLM-powered VA in section \ref{sec:results-chatGPT-breakdowns}  and as discussed above in sections \ref{sec:discussion-levraging-llm} and \ref{sec:discussion-speech-challenges}. 
%Recent work has also shown potential and benefits of LLMs in improving intent recognition to reduce conversational breakdowns \cite{mahmood2023llm}. 

\begin{adjustwidth}{0.3cm}{0pt}

    
    \textbf{Limitation 6:}
    \textit{Lack of VAs' comprehension of naturalistic and diverse speech styles leads to conversational breakdowns and subpar user experience\cmh{didn't we discuss this before?}.}

    \noindent
    \hl{\textbf{Design Consideration 9:}
    \textit{Design VAs to be human-aware to detect their implicit intent through verbal and vocal cues.}}

    \noindent
    \hl{\textbf{Design Consideration 10:}
    \textit{Enhance VAs' natural speech comprehension using LLMs' contextual understanding for improved user interactions.}}\cmh{didn't we discuss this before?}
  


\end{adjustwidth}     

\begin{comment}
    


\subsection{Design Considerations for LLM-powered VAs for Older Adults}
In exploring the interactions of older adults with LLM-powered VAs, our findings provide insights into such VAs' conversational capabilities and resilience to errors. Based on these insights we highlight opportunities, challenges, and provide design considerations for future LLM-powered conversational VAs for older adults. 

\subsubsection{Enhanced VA conversational capabilities and older adults learning curve}

The integration of LLMs into VAs significantly enhances their conversational abilities for information retrieval. Such LLM-powered VA maintains context and conversational history, enabling users, to ask follow-up questions and engage in multi-turn interactions with reduced friction \cite{mahmood2023llm}. 
For example, P15 demonstrated such enhanced interaction by asking a follow-up question, ``Why should I keep the room dark,'' after receiving the said advice on falling asleep (refer to C16 in Table \ref{tab:alexa-dialogue-chatGPT}). This ability to maintain context and respond to vague, more conversational queries represents a substantial improvement in VA-user interaction for older adults.

Additionally, our observations indicate that older adults, such as P15, become more adept at interacting with the ChatGPT-powered Alexa with practice. Comparing P15's initial interaction in the afternoon (C15 in Table \ref{tab:alexa-dialogue-chatGPT}) with a later one in the evening of the same day (C17 in Table \ref{tab:alexa-dialogue-chatGPT}) reveals a more fluid conversation, suggesting a learning curve. Improvement after trial and error in user interaction with such advanced VAs highlights the critical role of guidance for older adults in their initial usage stages. To facilitate this familiarization process and improve their overall experience, it is beneficial for VAs to provide instructive tutorials and helpful tips during interactions. For example, incorporating suggestions like, ``By the way, you can ask me follow-up questions without having to say the keyword,'' or informative prompts such as, ``I can answer any questions regarding history, technology, and can fetch recipes,'' can significantly aid users in understanding the breadth and depth of the VA's capabilities. Such approach not only makes the technology more accessible but also empowers users to make the most of their VA interactions.

\begin{adjustwidth}{0.3cm}{0pt}

    
    \textbf{Opportunity 2:}
    \textit{LLM-powered VAs can enhance older adults experience for information retrieval.}

    \noindent
    \textbf{Opportunity 3:}
    \textit{Learning curve in older adults using advanced VAs reveals an opportunity to enhance user experience through trial and error.}
    
    \noindent
    \hl{\textbf{Design Consideration 7:}
    \textit{Embed instructive tutorials and tips in VA interactions to help older adults effectively use advanced voice assistant features.}}  


\end{adjustwidth}   


 

\subsubsection{Conversational resilience}
\label{sec:discussion-LLM-conversational resilience}
%Seamless integration is essential for older adults using VAs, as our study shows that additional steps for skill activation can act as barriers for adoption and use of ChatGPT-powered Alexa skill. Most errors in these interactions were noted at the skill activation level, particularly during attempts to exit the skill (section \ref{sec:results-chatGPT-breakdowns}). To improve user experience, VAs should not require explicit activation and should use natural language for skill closure and termination to enable more intuitive and user-friendly interactions, specifically since older adults tend to be forgetful as discussed in section\ref{sec:discussion-forgetfulness}.


%In interactions involving ChatGPT, we observed that all intent recognition errors were regarding the misinterpreting users' intent to exit the Alexa skill rather than ChatGPT's understanding of user intent, indicating ChatGPT's high level of accuracy in understanding user requests. 
In interactions with ChatGPT, all intent recognition errors related to misinterpreting participant intent to exit the Alexa skill, not ChatGPT's understanding of their intent, highlighting its high accuracy in comprehending user requests.
Most errors were related to Alexa's speech technology and skill activation level, particularly during attempts to exit the skill, yet the overall intent was accurately identified in most cases (see section \ref{sec:results-chatGPT-breakdowns}). Notably,  errors in ChatGPT skill interactions were often resolved within a maximum of two retry attempts by participants, showcasing better error resolution compared to standard Alexa interactions where many errors remained unresolved despite multiple retries as shown in section \ref{sec:errors-retry}.

However, we identified issue of partial listening errors, particularly prevalent among older adults as they may take longer to formulate their queries (C13 Table \ref{tab:alexa-dialogue-chatGPT})---suggesting a need for improvement in Alexa's voice interface to better accommodate users with slower speech patterns and speech difficulties.%, as illustrated in conversation 
Given that interactions with LLM-integrated VAs tend to be more conversational and the responses more verbose \cite{mahmood2023llm}, it is crucial for these systems to allow ample time for users, especially older adults, to process the information and articulate their queries. Adaptions to user speech rate and context would ensure that voice user interfaces (VUIs) are more aligned with the communication styles and needs of older users, enhancing the overall usability and effectiveness of the technology.





\begin{adjustwidth}{0.3cm}{0pt}

    
    \textbf{Opportunity 4:}
    \textit{Enhanced error resolution and intent recognition in VAs with LLM integration can be beneficial for older users.}

    \noindent
    \textbf{Limitation 6:}
    \textit{Limited adaptability of VUIs for current assistants to slower speech patterns and extended speaking time needs of older adults especially when VAs are more conversational.}
    
    \noindent
    \hl{\textbf{Design Consideration 8:}
    \textit{Tailor VUIs to better suit the conversational pace and preferences of older adults, ensuring more fluid conversational interaction.}}  


\end{adjustwidth}   

%\subsubsection{Purpose-driven LLM-powered VAs}
\end{comment}


==> conversations.tex <==
\begin{table}[h]
\centering
\caption{Example conversations of  ``\dots'' represents truncation of conversation for brevity.  Full conversations are presented in supplementary materials.}
\label{tab:alexa-dialogue}
\begin{tabular}{p{0.3cm} M L}
%\hline
\textbf{Tag} & \textbf{Participant} & \textbf{Alexa} \\
\midrule
\midrule
C1 & What are Joe Biden's roots? & According to an Alexa Answers contributor: Ireland\\
\cdashline{2-3}
P2 & Alexa that's his lineage I wanna know about his mother and his father & [not listened by Alexa] \\
 \cdashline{2-3}
 & Alexa tell me about virus family his parents. \myc{[Transcription error, he actually said: Alexa tell me about Joe Biden's family his parents] }& From cdc.gov: Mayaro virus (MAYV), the cause of Mayaro fever, is a member of the genus Alphavirus, family Togaviridae, and is closely related to Chikungunya, O’nyong-nyong, Ross River, Barmah Forest, and Sindbis viruses (1–3). \\
 \cdashline{2-3}
 & Alright Alexa you did a really good job at answering question I did not ask you & \myc{[not listened by Alexa]} \\
 \cdashline{2-3}
 & Alexa tell me about Joe Biden's family his mother his father & Joe Biden's children are Ashley Biden, Beau Biden, Hunter Biden, and Naomi Biden. His parent is Jean Biden, his siblings are Francis Biden, James Biden, and Valerie Biden Owens, and his relative is Valerie Biden Owens. \\
 \cdashline{2-3}
 & Alexa show his mother was a single mother \myc{[Transcription error he actually said: Alexa so his mother is a single mother?]} & From educalingo.com: The definition of single mother in the dictionary is a mother who has a dependent child or dependent children and who is widowed, divorced, or unmarried. \\
 \cdashline{2-3}
 & Alexa Joe Biden's family was did he have a father than you & Joe Biden's father is Joseph R. Biden Sr.. \\
 \cdashline{2-3}
 & What did he do? & \myc{[not listened by Alexa]} \\
 \cdashline{2-3}
 & Alexa what was Joe Biden senior's educational background and what did he do? & This might answer your question: Joe Biden was educated at Syracuse University and the University of Delaware. \\
 \cdashline{2-3}
 & Alexa what was Joe Biden's father's background? & Hmm, I don't know that one. \\
 \cdashline{2-3}
 & Alexa did Joe Biden know his father & Joe Biden's father is Joseph R. Biden Sr.. \\
 \cdashline{2-3}
 & What what was Joseph F. Biden's educational background? & Before his political career, former Vice President Joe Biden was an attorney. In 1965, he received a bachelor's degree in history and political science from the University of Delaware. In 1968, Biden earned his juris doctors degree from Syracuse University College of Law. \\
 \cdashline{2-3}
 & Alexa stop I'm talking about Joe Biden's father what was his educational background & Sorry, I don't know that one \\
 \cdashline{2-3}
%\cline{2-3}
%& Conversation3 & Pattern3 \\
\hline
C2 & Alexa I've got a math problem what is the likelihood today June the twenty fourth that I will get one hour straight sun
& In [city], at 11:00 AM, it'll be 76 degrees Fahrenheit with cloudy skies. At 12:00 PM, it'll be 78 degrees with cloudy skies. At 1:00 PM, it'll be 80 degrees with cloudy skies. At 2:00 PM, it'll be 80 degrees with thunderstorms and mostly cloudy skies.  \\ 
\cdashline{2-3}
P2 & Alexa you did not answer the math question the answer should come in percentage &  In [city], at 11:00 AM, it'll be 76 degrees Fahrenheit with cloudy skies. At 12:00 PM, it'll be 78 degrees with cloudy skies. At 1:00 PM, it'll be 80 degrees with cloudy skies. At 2:00 PM, it'll be 80 degrees with thunderstorms and mostly cloudy skies. \\
\hline

%\multirow{2}{*}{Tag2} & Conversation4 & Pattern4 \\
%\cline{2-3}
%& Conversation5 & Pattern5 \\
%\hline
\end{tabular}
\end{table}


\begin{table}[h]
\centering
\caption{Example conversations related to errors.  ``\dots'' represents truncation of conversation for brevity.  }
\label{tab:alexa-dialogue-errors}
\begin{tabular}{p{0.3cm} M L}
%\hline
\textbf{Tag} & \textbf{Participant} & \textbf{Alexa} \\
\midrule
\midrule
C9 \newline P2 & Alexa in the most recent literature produced by the FDA what kind of cancer did Aspartame causes? & According to Mayo Clinic: Cancer is caused by changes, or mutations, to the DNA \dots \myc{[intent error]}\\% within your cells. The DNA inside a cell is packaged into a large number of genes. Each gene contains a set of instructions that tells the cell what to do. Mistakes in the instructions sometimes allow a cell to become cancerous. Gene mutations can be inherited from your parents. But most of these changes occur throughout life, in response to outside factors like smoking, radiation, viruses, and lack of exercise.\\
 & Alexa, you're a circular idiot & \myc{[No response from Alexa]} \\ 
 \hline
C10 & Alexa, tell me something wonderful & I wasn't able to understand the question I heard \myc{[limitation error]}. \\ %University of Pennsylvania.	\\
\cdashline{2-3}
P11a & It's ok \myc{[laughter]} It's amazing & Great! \myc{[It's amazing not listened by Alexa]} \\
 \hline
C11 & Alexa I took my medicine  & Sorry, I don't know that \myc{[intent error]} \\ %University of Pennsylvania.	\\
\cdashline{2-3}
P15 & Yes I took my medicine &  Hmm, I don't know that one. \myc{[intent error]}\\
 \hline
 & Cancel medicine  & \{P15's name\}, I can’t find medicine, what's the date or time of the event you want to delete? \myc{[intent error]}\\ %University of Pennsylvania.	\\
\cdashline{2-3}
 & Cancel the alert & \myc{[reminder stops ringing]}  \\

 
 \hline

\end{tabular}
\end{table}


\begin{table}[h]
\centering
\caption{Example conversations of social aspects beyond simple interactions.  ``\dots'' represents truncation of conversation for brevity.  Full conversations are presented in supplementary materials.}
\label{tab:alexa-dialogue-private-conversations}
\begin{tabular}{p{0.3cm} M L}
%\hline
\textbf{Tag} & \textbf{Participant} & \textbf{Alexa} \\
\midrule
\midrule

C3 & Alexa what is Donald Trump's educational background? & Donald Trump was educated at the UPenn. \\ %University of Pennsylvania.	\\
\cdashline{2-3}
P2 & That's it, no Harvard no Yale. \myc{[remark]} & \myc{[not listened by Alexa]} \\
 \hline
C4 & \myc{[User initiates incomplete reminder request]} & When should I remind you? \\% and is closely related to Chikungunya, O’nyong-nyong, Ross River, Barmah Forest, and Sindbis viruses (1–3). \\
 \cdashline{2-3}
P11b & \myc{[No user response]} & What's the reminder for? \\
 \cdashline{2-3}
 & She Remembers it! & \\%, James Biden, and Valerie Biden Owens, and his relative is Valerie Biden Owens. \\
 \hline
C5 & Alexa put hard candy on my shopping list.  & You already have hard candy on your shopping list. \\ %University of Pennsylvania.	\\
\cdashline{2-3}
P6 & Oh. Did you hear her? I said Alexa \dots \myc{[P6 to visitor]}&  \\
 \hline
C6 & Alexa, give me a 10 minute warning please.  & 10 minutes, starting now \\ %University of Pennsylvania.	\\
\cdashline{2-3}
P11a & & \cellcolor{user} \myc{[P11b to P11a:} No you need to say timer for 10 minutes \myc{[overlapping Alexa speech]}  \\
\cdashline{2-3}
 & What wait wait what \{P11b's name\} & \cellcolor{user} \myc{[P11b to P11a]:} Set a time for 10 minutes  \\
 \cdashline{2-3}
 & Okay \myc{[To P11b]} Alexa, set timer for 10 minutes & Second timer, 10 minutes, starting now \\
 \cdashline{2-3}
 & Set a time for 10 minutes \myc{[P11b to P11a]} & \\
 \cdashline{2-3}
C7 & Alexa add milk to my shopping list.  & I added milk to your Shopping list. \\ %University of Pennsylvania.	\\
\cdashline{2-3}
P8 & I don't know where the list is. Oh wait a minute may be it's in Amazon. \dots \myc{[Visitor to P8]} &  \\
 \hline
C8 & Alexa, give me a 10 minute warning please.  & 10 minutes, starting now \\ %University of Pennsylvania.	\\
\cdashline{2-3}
P11a & Alexa play the history of Tony Bennett.& \cellcolor{user} \myc{[P11b to P11a]:} What's the history of Tony Bennett  \\
\cdashline{2-3}
 & \myc{[To P11b]} Oh she'll tell you & \cellcolor{user} \myc{[P11b chuckles mockingly]} \\
 \cdashline{2-3}
 & She didn't tell you \myc{[to P11b]}  & \cellcolor{user} \myc{[P11b to P11a]:} Because it makes no sense\\
 \cdashline{2-3}
 
 \hline

\end{tabular}
\end{table}
